Towards Multimodal Depth Estimation from Light Fields

Light field applications, especially light field rendering and depth estimation, developed rapidly in recent years. While state-of-the-art light field rendering methods handle semi-transparent and reflective objects well, depth estimation methods either ignore these cases altogether or only deliver a weak performance. We argue that this is due current methods only considering a single "true" depth, even when multiple objects at different depths contributed to the color of a single pixel. Based on the simple idea of outputting a posterior depth distribution instead of only a single estimate, we develop and explore several different deep-learning-based approaches to the problem. Additionally, we contribute the first "multimodal light field depth dataset" that contains the depths of all objects which contribute to the color of a pixel. This allows us to supervise the multimodal depth prediction and also validate all methods by measuring the KL divergence of the predicted posteriors. With our thorough analysis and novel dataset, we aim to start a new line of depth estimation research that overcomes some of the long-standing limitations of this field.

==> Towards Multimodal Depth Estimation from Light Fields/figures/architectures/base.tex <==
\begin{tikzpicture}[
    data domain/.style={fill=black!20, draw=black, rounded corners=3pt, minimum height=3.15em, minimum width=1.5em, align=center, font=\normalsize},
    half data domain/.style={fill=black!20, draw=black, rounded corners=3pt, minimum height=1.5em, minimum width=1.33em, align=center, font=\normalsize},
    fat arrow/.style={double arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=3em, text=black!5},
    unidirectional fat arrow/.style={single arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=4em, text=black!5},
    loss/.style={black!75, midway, align=center, font=\footnotesize\sffamily\bfseries}]

    \node [data domain, fill=black!5] (x) {$x$};
    \node [below=6pt of x.south, yshift=5pt] (inp) {\normalsize{\textsc{Light Field}}};

    \node [unidirectional fat arrow, right=4pt of x.east] (cnn) {\textsf{\normalsize{\textbf{CNN}}}};
    \node [data domain, fill=black!5, right=2pt of cnn.east, fill=my-orange!30] (y) {$\hat y$};
    \node [below=6pt of y.south, yshift=5pt] (out) {\normalsize{\textsc{Disparity}}};
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/figures/architectures/dpp.tex <==
\begin{tikzpicture}[
    data domain/.style={fill=black!20, draw=black, rounded corners=3pt, minimum height=3.15em, minimum width=1.5em, align=center, font=\normalsize},
    fat arrow/.style={double arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=3em, text=black!5},
    unidirectional fat arrow/.style={single arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=4em, text=black!5},
    loss/.style={black!75, midway, align=center, font=\normalsize\sffamily\bfseries}]

    \node [data domain, fill=black!5] (x) {$x$};
    \node [below=6pt of x.south, yshift=5pt] (inp) {\normalsize{\textsc{Light Field}}};

    \node [unidirectional fat arrow, right=2pt of x.east] (INN) {\textsf{\normalsize{\textbf{CNN}}}};

    \node [data domain, right=2pt of INN.east, fill=my-blue!30] (z) {$z$};
    \node [below=6pt of z.south, yshift=5pt] (gmm) {\normalsize{\textsc{Scores}}};
    
    \node [unidirectional fat arrow, right=4pt of z.east] (inference) {\textsf{\normalsize{\textbf{Softmax}}}};
    
    \node [data domain, right=2pt of inference.east, fill=my-purple!30] (y) {$p(y \! \mid \! x)$};
    \node [below=6pt of y.south, yshift=5pt] (output) {\normalsize{\textsc{Posterior}}};
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/figures/architectures/ese.tex <==
\begin{tikzpicture}[
    data domain/.style={fill=black!20, draw=black, rounded corners=3pt, minimum height=3.15em, minimum width=1.5em, align=center, font=\normalsize},
    half data domain/.style={fill=black!20, draw=black, rounded corners=3pt, minimum height=1.5em, minimum width=1.8em, align=center, font=\normalsize},
    fat arrow/.style={double arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=3em, text=black!5},
    unidirectional fat arrow/.style={single arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=4em, text=black!5},
    unidirectional fat short arrow/.style={single arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=1.5em, text=black!5},
    loss/.style={black!75, midway, align=center, font=\normalsize\sffamily\bfseries}]
    
    \foreach \i/\y in {0/0,1/-2.25,2/-4.5}
    {
        \node [data domain, fill=black!5] (x) at (0, \y) {$x_{\i}$};

        \node [unidirectional fat arrow, right=4pt of x.east] (cnn) {\textsf{\normalsize{\textbf{CNN}}}};

        \node [half data domain, above right=0.5pt of cnn.east, fill=my-orange!30] (mu) {$\mu_{\i}$};
        \node [half data domain, below right=0.5pt of cnn.east, fill=my-green!30] (sigma) {$b_{\i}$};
        
        \node [unidirectional fat short arrow, below=9pt of x.south, rotate=-90, xshift=4pt, yshift=6.375pt] (shift) {\textsf{\scriptsize{\textbf{Shift}}}};
        
        \node [below=6pt of sigma.south, yshift=5pt] (out) {\normalsize{\textsc{Laplacian}}};
    }
    
    \node [below=25pt of x.south, yshift=-5pt, xshift=0.75pt] (inp) {\dots};

    %\node [below=20pt of x.south, yshift=5pt] (inp) {\tiny{\textsc{Light Field}}};
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/figures/architectures/ib-inn.tex <==
\begin{tikzpicture}[
    data domain/.style={fill=black!20, draw=black, rounded corners=3pt, minimum height=3.15em, minimum width=1.5em, align=center, font=\normalsize},
    fat arrow/.style={double arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=3em, text=black!5},
    unidirectional fat arrow/.style={single arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=4em, text=black!5},
    loss/.style={black!75, midway, align=center, font=\footnotesize\sffamily\bfseries}]

    \node [data domain, fill=black!5] (x) {$x$};
    \node [below=6pt of x.south, yshift=5pt] (inp) {\normalsize{\textsc{Light Field}}};

    \node [fat arrow, right=2pt of x.east] (INN) {\textsf{\normalsize{\textbf{INN}}}};

    \node [data domain, right=2pt of INN.east, fill=my-blue!30] (z) {$z$};
    \node [below=6pt of z.south, yshift=5pt] (gmm) {\normalsize{\textsc{GMM}}};
    
    \node [unidirectional fat arrow, right=4pt of z.east] (inference) {\textsf{\scriptsize{\textbf{Bayes Rule}}}};
    
    \node [data domain, right=2pt of inference.east, fill=my-purple!30] (y) {$p(y \! \mid \! x)$};
    \node [below=6pt of y.south, yshift=5pt] (output) {\normalsize{\textsc{Posterior}}};
\end{tikzpicture}


==> Towards Multimodal Depth Estimation from Light Fields/figures/architectures/upr.tex <==
\begin{tikzpicture}[
    data domain/.style={fill=black!20, draw=black, rounded corners=3pt, minimum height=3.15em, minimum width=1.5em, align=center, font=\normalsize},
    half data domain/.style={fill=black!20, draw=black, rounded corners=3pt, minimum height=1.5em, minimum width=1.33em, align=center, font=\normalsize},
    fat arrow/.style={double arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=3em, text=black!5},
    unidirectional fat arrow/.style={single arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=4em, text=black!5},
    loss/.style={black!75, midway, align=center, font=\footnotesize\sffamily\bfseries}]

    \node [data domain, fill=black!5] (x) {$x$};
    \node [below=6pt of x.south, yshift=5pt] (inp) {\normalsize{\textsc{Light Field}}};

    \node [unidirectional fat arrow, right=4pt of x.east] (cnn) {\textsf{\normalsize{\textbf{CNN}}}};
    \node [half data domain, above right=0.5pt of cnn.east, fill=my-orange!30] (mu) {$\mu$};
    \node [half data domain, below right=0.5pt of cnn.east, fill=my-green!30] (sigma) {$b$};
    \node [below=6pt of sigma.south, yshift=5pt] (out) {\normalsize{\textsc{Laplacian}}};
\end{tikzpicture}


==> Towards Multimodal Depth Estimation from Light Fields/figures/bimodality/cnn.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{$1 - \mathrm{\textsc{\textsc{Intersection}}}$},
        xlabel=\scriptsize{\textsc{Fraction of Predicted Pixels}},
        ]
    
        %\addplot[mark=none, black!80, thick] 
        %table[x=frac,y=uncert,col sep=comma] {figures/bimodality/random.csv}; 
        
        \addplot[mark=none, my-orange, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality/bayesian.csv};
        
        \addplot[mark=none, my-purple, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality/discrete.csv};
        
        \addplot[mark=none, my-green, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality/ib-inn.csv}; 

        \addplot[mark=none, black!80, thick, densely dotted]
        table[x=frac,y=oracle,col sep=comma] {figures/bimodality/ib-inn.csv}; 
        
        %\addlegendentry{\scriptsize{Random}}
        \addlegendentry{\scriptsize{ESE}}
        \addlegendentry{\scriptsize{DPP}}
        \addlegendentry{\scriptsize{IB-INN}}
        \addlegendentry{\scriptsize{Oracle}}
    \end{axis}
\end{tikzpicture}


==> Towards Multimodal Depth Estimation from Light Fields/figures/bimodality/error.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{\textsc{Bimod. $-$ Oracle}},
        xlabel=\scriptsize{\textsc{Fraction of Predicted Pixels}},
        ]
        
        %\addplot[mark=none, my-blue, thick] 
        %table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality/random.csv}; 

        \addplot[mark=none, my-orange, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality/bayesian.csv}; 
        
        \addplot[mark=none, my-purple, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality/discrete.csv};

        \addplot[mark=none, my-green, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality/ib-inn.csv};
    
        %\addlegendentry{\scriptsize{Random}}
        \addlegendentry{\scriptsize{ESE}}
        \addlegendentry{\scriptsize{DPP}}
        \addlegendentry{\scriptsize{IB-INN}}
        
    \end{axis}
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/figures/bimodality_betas/cnn.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        ymin=-0.1,
        ymax=1.6,
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{$1 - \mathrm{\textsc{\textsc{Intersection}}}$},
        xlabel=\scriptsize{\textsc{Fraction of Predicted Pixels}},
        ]
    
        %\addplot[mark=none, black!80, thick] 
        %table[x=frac,y=uncert,col sep=comma] {figures/bimodality/random.csv}; 
        
        \addplot[mark=none, my-orange, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality_betas/0.csv};
        
        \addplot[mark=none, my-purple, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality_betas/1.csv};
        
        \addplot[mark=none, my-green, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality_betas/2.csv}; 

        \addplot[mark=none, my-blue, thick]
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality_betas/4.csv}; 
        
        \addplot[mark=none, red!80, thick]
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality_betas/8.csv}; 
        
        \addplot[mark=none, black!80, thick, densely dotted]
        table[x=frac,y=oracle,col sep=comma] {figures/bimodality_betas/8.csv}; 
        
        %\addlegendentry{\scriptsize{Random}}
        \addlegendentry{\scriptsize{$\beta = 0$}}
        \addlegendentry{\scriptsize{$\beta = 1$}}
        \addlegendentry{\scriptsize{$\beta = 2$}}
        \addlegendentry{\scriptsize{$\beta = 4$}}
        \addlegendentry{\scriptsize{$\beta = 8$}}
        \addlegendentry{\scriptsize{Oracle}}
    \end{axis}
\end{tikzpicture}


==> Towards Multimodal Depth Estimation from Light Fields/figures/bimodality_betas/error.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        ymin=-0.1,
        ymax=1.1,
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{\textsc{Bimod. $-$ Oracle}},
        xlabel=\scriptsize{\textsc{Fraction of Predicted Pixels}},
        ]
        
        \addplot[mark=none, my-orange, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality_betas/0.csv};
        
        \addplot[mark=none, my-purple, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality_betas/1.csv};
        
        \addplot[mark=none, my-green, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality_betas/2.csv}; 

        \addplot[mark=none, my-blue, thick]
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality_betas/4.csv}; 
        
        \addplot[mark=none, red!80, thick]
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality_betas/8.csv}; 
        
        %\addlegendentry{\scriptsize{Random}}
        \addlegendentry{\scriptsize{$\beta = 0$}}
        \addlegendentry{\scriptsize{$\beta = 1$}}
        \addlegendentry{\scriptsize{$\beta = 2$}}
        \addlegendentry{\scriptsize{$\beta = 4$}}
        \addlegendentry{\scriptsize{$\beta = 8$}}
    \end{axis}
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/figures/posteriors/bimodal.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.694\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.2)}},
        y label style={at={(axis description cs:0.2,0.5)}},
        ylabel=$p(y | x)$,
        xlabel=disparity $y$,
        xmin=-1,
        xmax=0.5,
        %ymin=-0.1,
        %ymax=2.1,
        yticklabels={,,},
        xticklabels={,,},
        ]

        \addplot[mark=none, my-green, thick] 
        table[x=y,y=p,col sep=comma] {figures/posteriors/posterior_bm_pred.csv}; 

        \addplot[mark=none, my-orange, thick] 
        table[x=y,y=p,col sep=comma] {figures/posteriors/posterior_bm_inn.csv}; 

        \addlegendentry{\scriptsize{Predictive}}
        \addlegendentry{\scriptsize{IB-INN}}
    \end{axis}
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/figures/posteriors/unimodal.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.694\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1, at={(0.02,0.02)},anchor=south west},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.2)}},
        y label style={at={(axis description cs:0.2,0.5)}},
        ylabel=$p(y | x)$,
        xlabel=disparity $y$,
        xmin=0.0,
        xmax=1.0,
        %ymin=-0.1,
        %ymax=2.1,
        yticklabels={,,},
        xticklabels={,,},
        ]

        \addplot[mark=none, my-green, thick] 
        table[x=y,y=p,col sep=comma] {figures/posteriors/posterior_um_pred.csv}; 

        \addplot[mark=none, my-orange, thick] 
        table[x=y,y=p,col sep=comma] {figures/posteriors/posterior_um_inn.csv};

        \addlegendentry{\scriptsize{Predictive}}
        \addlegendentry{\scriptsize{IB-INN}}
    \end{axis}
\end{tikzpicture}


==> Towards Multimodal Depth Estimation from Light Fields/figures/results_posteriors/0007_multi/posteriors.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.422\linewidth,
        legend cell align={left},
        grid=major,
        grid style={densely dotted, gray!50},
        legend style={fill=white, fill opacity=1, draw opacity=1,text opacity=1},
        x label style={at={(axis description cs:0.5,0.07)}},
        y label style={at={(axis description cs:0.07,0.5)}},
        ybar interval,
        % bar width=3,
        ylabel=$p(y | x)$,
        xlabel=discretized disparity $y$,
        xmin=1.5,
        xmax=2.5,
        xticklabels={,,},
        yticklabels={,,},
        ]
        
        \addplot[mark=none, my-orange, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0007_multi/upr.csv};
        
        \addplot[mark=none, my-green, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0007_multi/dpp.csv}; 
        
        \addplot[mark=none, my-blue, fill] 
        table[x=y,y=gt,col sep=comma] {figures/results_posteriors/0007_multi/upr.csv}; 
        
        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{DPP}}
        \addlegendentry{\scriptsize{GT}}
    \end{axis}
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/figures/results_posteriors/0007_uni/posteriors.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.422\linewidth,
        legend cell align={left},
        grid=major,
        grid style={densely dotted, gray!50},
        legend style={fill=white, fill opacity=1, draw opacity=1,text opacity=1},
        x label style={at={(axis description cs:0.5,0.07)}},
        y label style={at={(axis description cs:0.07,0.5)}},
        ybar interval,
        % bar width=3,
        ylabel=$p(y | x)$,
        xlabel=discretized disparity $y$,
        xmin=1.5,
        xmax=2.5,
        xticklabels={,,},
        yticklabels={,,},
        ]
        
        \addplot[mark=none, my-orange, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0007_uni/upr.csv};
        
        \addplot[mark=none, my-green, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0007_uni/dpp.csv}; 
        
        \addplot[mark=none, my-blue, fill] 
        table[x=y,y=gt,col sep=comma] {figures/results_posteriors/0007_uni/upr.csv}; 
        
        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{DPP}}
        \addlegendentry{\scriptsize{GT}}
    \end{axis}
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/figures/results_posteriors/0013_uni/posteriors.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.422\linewidth,
        legend cell align={left},
        grid=major,
        grid style={densely dotted, gray!50},
        legend style={fill=white, fill opacity=1, draw opacity=1,text opacity=1},
        x label style={at={(axis description cs:0.5,0.07)}},
        y label style={at={(axis description cs:0.07,0.5)}},
        ybar interval,
        % bar width=3,
        ylabel=$p(y | x)$,
        xlabel=discretized disparity $y$,
        xmin=1.2,
        xmax=2.2,
        xticklabels={,,},
        yticklabels={,,},
        ]
        
        \addplot[mark=none, my-orange, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0013_uni/upr.csv};
        
        \addplot[mark=none, my-green, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0013_uni/dpp.csv}; 
        
        \addplot[mark=none, my-blue, fill] 
        table[x=y,y=gt,col sep=comma] {figures/results_posteriors/0013_uni/upr.csv}; 
        
        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{DPP}}
        \addlegendentry{\scriptsize{GT}}
    \end{axis}
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/figures/results_posteriors/0123_multi/posteriors.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.422\linewidth,
        legend cell align={left},
        grid=major,
        grid style={densely dotted, gray!50},
        legend style={fill=white, fill opacity=1, draw opacity=1,text opacity=1},
        x label style={at={(axis description cs:0.5,0.07)}},
        y label style={at={(axis description cs:0.07,0.5)}},
        ybar interval,
        % bar width=3,
        ylabel=$p(y | x)$,
        xlabel=discretized disparity $y$,
        xmin=1,
        xmax=3.75,
        xticklabels={,,},
        yticklabels={,,},
        ]
        
        \addplot[mark=none, my-orange, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0123_multi/upr.csv};
        
        \addplot[mark=none, my-green, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0123_multi/dpp.csv}; 
        
        \addplot[mark=none, my-blue, fill] 
        table[x=y,y=gt,col sep=comma] {figures/results_posteriors/0123_multi/upr.csv}; 
        
        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{DPP}}
        \addlegendentry{\scriptsize{GT}}
    \end{axis}
\end{tikzpicture}


==> Towards Multimodal Depth Estimation from Light Fields/figures/results_posteriors/0123_uni/posteriors.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.422\linewidth,
        legend cell align={left},
        grid=major,
        grid style={densely dotted, gray!50},
        legend style={fill=white, fill opacity=1, draw opacity=1,text opacity=1},
        x label style={at={(axis description cs:0.5,0.07)}},
        y label style={at={(axis description cs:0.07,0.5)}},
        ybar interval,
        % bar width=3,
        ylabel=$p(y | x)$,
        xlabel=disparity $y$,
        xmin=1,
        xmax=3.75,
        xticklabels={,,},
        yticklabels={,,},
        ]
        
        \addplot[mark=none, my-orange, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0123_uni/upr.csv};
        
        \addplot[mark=none, my-green, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0123_uni/dpp.csv}; 
        
        \addplot[mark=none, my-blue, fill] 
        table[x=y,y=gt,col sep=comma] {figures/results_posteriors/0123_uni/upr.csv}; 
        
        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{DPP}}
        \addlegendentry{\scriptsize{GT}}
    \end{axis}
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/figures/sparsify/cnn.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{\textsc{BadPix (normalized)}},
        xlabel=\scriptsize{\textsc{Fraction of Removed Pixels}},
        ]

        \addplot[mark=none, my-blue, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/sparsify/upr.csv}; 

        \addplot[mark=none, my-blue, thick, densely dotted]
        table[x=frac,y=oracle,col sep=comma] {figures/sparsify/upr.csv}; 
        
        % \addplot[mark=none, my-orange, thick, densely dotted] 
        % table[x=frac,y=uncert,col sep=comma] {figures/sparsify/random.csv};

        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{Oracle}}
        % \addlegendentry{\scriptsize{Random}}
    \end{axis}
\end{tikzpicture}


==> Towards Multimodal Depth Estimation from Light Fields/figures/sparsify/error.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{\textsc{Sparsif. $-$ Oracle}},
        xlabel=\scriptsize{\textsc{Fraction of Removed Pixels}},
        ]

        \addplot[mark=none, my-blue, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/sparsify/upr.csv}; 
        
        \addplot[mark=none, my-orange, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/sparsify/ese.csv}; 
        
        \addplot[mark=none, my-purple, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/sparsify/dpp.csv};

        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{ESE}}
        \addlegendentry{\scriptsize{DPP}}
    \end{axis}
\end{tikzpicture}


==> Towards Multimodal Depth Estimation from Light Fields/figures/sparsify_hci/cnn.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{\textsc{BadPix (normalized)}},
        xlabel=\scriptsize{\textsc{Fraction of Removed Pixels}},
        ]

        \addplot[mark=none, my-blue, thick]
        table[x=frac,y=uncert,col sep=comma] {figures/sparsify_hci/upr.csv}; 
        
        \addplot[mark=none, my-blue, thick, densely dotted]
        table[x=frac,y=oracle,col sep=comma] {figures/sparsify_hci/upr.csv}; 
        
        %\addlegendentry{\scriptsize{Random}}
        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{Oracle}}
    \end{axis}
\end{tikzpicture}


==> Towards Multimodal Depth Estimation from Light Fields/figures/sparsify_hci/error.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{\textsc{Sparsif. $-$ Oracle}},
        xlabel=\scriptsize{\textsc{Fraction of Removed Pixels}},
        ]

        \addplot[mark=none, my-blue, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/sparsify_hci/upr.csv};
        
        \addplot[mark=none, my-orange, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/sparsify_hci/ese.csv};
        
        \addplot[mark=none, my-purple, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/sparsify_hci/dpp.csv}; 
        
        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{ESE}}
        \addlegendentry{\scriptsize{DPP}}
    \end{axis}
\end{tikzpicture}


==> Towards Multimodal Depth Estimation from Light Fields/figures/square_pixel/square_pixel.tex <==
\begin{tikzpicture}
    \fill[my-orange] (0, 0) rectangle (\linewidth, \linewidth);
    \fill[my-blue] (0, 0) -- (0.3\linewidth, 0) -- (0.7\linewidth, \linewidth) -- (0, \linewidth);
    \draw[thick] (0.3\linewidth, 0) -- (0.7\linewidth, \linewidth);
    \draw[thick] (0, 0) rectangle (\linewidth, \linewidth);
    
    \node at (0.25\linewidth, 0.5\linewidth) {\Large $y_{i1}$};
    \node at (0.75\linewidth, 0.5\linewidth) {\Large $y_{i2}$};
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/figures/teaser/teaser.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        grid=major,
        grid style={densely dotted, gray!50},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        x label style={at={(axis description cs:0.5,0.1)}},
        y label style={at={(axis description cs:0.125,0.5)}},
        ylabel=$p(y | x)$,
        xlabel=disparity $y$,
        xmin=-2,
        xmax=0.25,
        ymin=-0.1,
        ymax=3.6,
        yticklabels={,,},
        xticklabels={,,},
        ]
        
        \addplot[mark=none, my-orange, thick] 
        table[x=y,y=p,col sep=comma] {figures/teaser/upr.csv};
        
        \addplot[mark=none, my-green, thick] 
        table[x=y,y=p,col sep=comma] {figures/teaser/ib-inn.csv}; 

        \addplot[mark=none, my-blue, thick] 
        table[x=y,y=p,col sep=comma] {figures/teaser/ground_truth.csv}; 
        
        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{ESE}}
        \addlegendentry{\scriptsize{GT}}
    \end{axis}
\end{tikzpicture}

==> Towards Multimodal Depth Estimation from Light Fields/sections/abstract.tex <==
% Image-based depth prediction methods developed rapidly in recent years.
% In particular, disparity estimation from light fields delivers superior results.
% Most remaining challenges occur in regions with multiple valid depth modes.
% Those multimodal cases include specular reflections, semi-transparent objects and depth edges.
% We address this by extending state-of-the-art methods to create four different posterior estimation approaches, based on feed-forward regression, ensembles and Invertible Neural Networks.
% A thorough evaluation of the predicted multimodal posterior distributions shows that the Invertible Neural Network performs accurately and efficiently in multimodal areas (\eg depth edges, semi-transparency).
% Methods that assume only one valid mode perform slightly better if this assumption holds.
% The contributed approaches can not only be used to sense depth through semi-transparent objects but may also contribute to future probabilistic depth estimation frameworks.
Light field applications, especially light field rendering and depth estimation, developed rapidly in recent years.
While state-of-the-art light field rendering methods handle semi-transparent and reflective objects well,
depth estimation methods either ignore these cases altogether or only deliver a weak performance.
We argue that this is due current methods only considering a single ``true'' depth, even when multiple objects at different depths contributed to the color of a single pixel.
Based on the simple idea of outputting a posterior depth distribution instead of only a single estimate, we develop and explore several different deep-learning-based approaches to the problem.
Additionally, we contribute the first ``multimodal light field depth dataset'' that contains the depths of all objects which contribute to the color of a pixel.
This allows us to supervise the multimodal depth prediction and also validate all methods by measuring the KL divergence of the predicted posteriors.
With our thorough analysis and novel dataset, we aim to start a new line of depth estimation research that overcomes some of the long-standing limitations of this field. 


==> Towards Multimodal Depth Estimation from Light Fields/sections/acknowledgement.tex <==
% !TEX root = ../paper.tex
We thank the Center for Information Services and High Performance Computing (ZIH) at TU Dresden for generous allocations of computer time.

==> Towards Multimodal Depth Estimation from Light Fields/sections/conclusion.tex <==
% !TEX root = ../paper.tex
%To summarize, we investigated posterior estimation methods for the exemplary task of depth from light fields.
%Specifically, we introduced and compared four approaches for multimodal depth estimation, building on common uncertainty quantification tools.
%This gives us valuable additional information in regions where the disparity could not be evaluated accurately before.
%We observe that methods assuming a unimodal posterior (\eg UPR) work best when this assumption holds.
%The IB-INN which predicts an arbitrary posterior distribution works best in multimodal areas.
To summarize: we investigated the problem of posterior estimation for dense regression on the exemplary task of depth estimation from light fields.
We therefore contributed the first light field dataset with multimodal depth ground truth.
Additionally, we introduced and compared novel approaches for multimodal light field depth estimation, building on common uncertainty quantification tools.
We observe that methods assuming a single valid depth work well if this assumption holds.
DPP, which predicts arbitrary posterior distributions, works best in general.
Our ESE method does not achieve the same performance, but estimates accurate confidence measures even for wide-baseline light fields.
We hope that our insights lay the foundations for a new line of depth estimation research that overcomes some long-standing limitations of the field.

==> Towards Multimodal Depth Estimation from Light Fields/sections/experiments.tex <==
% !TEX root = ../paper.tex
In this section, we describe our training procedure and analyze the predicted posterior distributions.
We therefore distinguish two possible applications: unimodal prediction with uncertainty and multimodal prediction.

\subsection{Architectures and Training Details}
\begin{figure}[t]
    \centering
    \begin{minipage}{.55\linewidth}
        \begin{subfigure}{\linewidth}
            \centering
            \resizebox{0.6\linewidth}{!}{\input{figures/architectures/base}}
            \subcaption{Baseline}
            \vspace{0.25cm}
        \end{subfigure}
        \begin{subfigure}{\linewidth}
            \centering
            \resizebox{0.6\linewidth}{!}{\input{figures/architectures/upr}}
            \subcaption{Unimodal Posterior Regression}
            \vspace{0.25cm}
        \end{subfigure}
        \begin{subfigure}{\linewidth}
            \resizebox{\linewidth}{!}{\input{figures/architectures/dpp}}
            \subcaption{Discrete Posterior Prediction}
        \end{subfigure}
        %\begin{subfigure}{\linewidth}
        %    \resizebox{\linewidth}{!}{\input{figures/architectures/ib-inn}}
        %    \subcaption{Information Bottleneck INN}
        %\end{subfigure}
    \end{minipage}
    \hfill
    \begin{minipage}{.4\linewidth}
        \begin{subfigure}{\linewidth}
            \vspace{-0.1cm}
            \resizebox{0.8\linewidth}{!}{\input{figures/architectures/ese}}
            \subcaption{EPI-Shift Ensemble}
        \end{subfigure}
    \end{minipage}
    \caption{
        \textbf{Network architecture overview:} 
        Our baseline is a simple feed-forward network trained to only predict disparity (a).
        We compare three posterior-regression methods:
        Laplacian prediction using learned loss attenuation (b), an ensemble on shifted inputs (d) and a discrete softmax classification network (c).
    }
    \label{fig:models}
    \vspace{-3mm}
\end{figure}
To ensure a fair comparison, we chose the state-of-the-art method EPI-Net~\cite{shin2018epinet} with minor modifications as our backbone network architecture for all models.
We describe the exact network architectures in more detail in~\cref{sec:architectures}.
The network consists of a total number of eight blocks, containing two convolutional layers, followed by a Rectified Linear Unit (ReLU) each and one Batch Normalization layer.
For UPR, we added an additional output layer to also predict the negative log width $-\log b$.
The EPI-Shift Ensemble is a modification of UPR with the only difference being the loss functions.
We experimented with different $\Delta y$ for our ESE method, resulting in different $M$s.
$\Delta y = 0.1$ performed best and gives $M = 70$ for the disparity range of our data.
Our extended EPI-Shift transformation, based on~\cite{leistner2019learning}, is described in more detail in~\cref{sec:epi-shift}.
%For the discrete methods we chose a number of `classes' equal to the number of input dimensions, thus the number of views times the number of color channels ($36 \times 3 = 108$).
For the discrete DPP method, we chose a number of $108$ ``classes''.
This is motivated by the common BadPix007 metric that consideres a pixel as ``correct'' if it is closer than $0.07\mathrm{px}$ to the ground truth.
A number of $108$ classes in a disparity range of $-3.5\dots3.5$ leads to a bin size of $\approx 0.065$ which is slightly below this threshold.
We implemented  our framework using PyTorch~\cite{paszke2019pytorch}.

We trained all networks using the loss functions described in \cref{sec:uncertainty}.
The unimodal loss functions, denoted as $\mathcal{L}_x$ are always applied to the closest disparity.
All multimodal loss functions, denoted as $\mathcal{L}_x^{\mathrm{MM}}$ are applied to all disparity modes.

In addition, we reimplemented EPI-Net~\cite{shin2018epinet} in our own framework as a baseline for a fair comparison.
The learning rate was set to $10^{-3}$ for all models, using a batch size of $512$ and the Adam optimizer.
We trained on randomly cropped patches ($96px \times 96px$) from the set of $100$ training scenes in our dataset.
To further improve the diversity of our dataset, we make use of a number of data augmentation operations:
We apply a random sub-pixel EPI-Shift between $-2\mathit{px}$ and $2\mathit{px}$~\cite{leistner2019learning}.
In addition, we randomly rotate the light field by a multiple of $90^\circ$, randomly rotate the colors in RGB-space and randomly change brightness and contrast.

\subsection{Posterior Evaluation}
%The performance of depth estimation methods is usually measured with a pixel-wise error to a ground truth disparity map. 
%But this alone is not sufficient for pixels with ambiguous depth.
%\Cref{fig:ground_truth} illustrates that the dataset ground truth is of limited use for multimodal pixels.
%This becomes clear at depth edges, where the color is a mixture of foreground and background colors.
%For synthetic scenes, this is caused by anti-aliasing during rasterization.
%In the real world, each pixel also captures the colors of multiple 3D points within a small angle, depending on the cameras Point Spread Function (PSF).
Depth estimation methods are usually evaluated by measuring the pixel-wise error to a ground truth disparity map.
However, to correctly measure the quality of estimates in areas with multiple valid depths, a different set of metrics is required.

We consider two application scenarios:
\textit{(i)} the estimation of just a single disparity, but with an additional confidence measure to ensure that the estimate can be ``trusted''.
This may be required, \eg in industrial and robotics applications where decisions are based on the estimated depth;
\textit{(ii)} the estimation of multiple depths in areas with transparent objects or at object edges.
This is typically required by Computer Graphics applications that aim to render the recorded scene from a different angle.
In the following, we introduce metrics for both cases.

%We argue, that for pixels that capture multiple depth modes, this is not sufficient.
%This occurs, for example, at depth edges:
%Each infinitesimally small point on the foreground and background object spreads across a finite area in the image plane, depending on the shape of the cameras PSF.
%This makes the separation of two closely projected points impossible~\cite{Kerviche2017}.
%As a consequence, pixels around depth edges always capture objects at multiple depths.
%\Cref{fig:ground_truth} illustrates that the dataset ground truth is of limited use for those pixels.
%Therefore, in order to measure the quality of posterior distribution predictions, we define and evaluate three separate tasks:

\subsubsection{Unimodal Prediction with Uncertainty}
\begin{figure*}[t]
    \centering
    \begin{subfigure}{0.495\textwidth}
        \resizebox{\linewidth}{!}{\input{figures/sparsify/cnn.tex}}
        \subcaption{Sparsification curve}
        \label{fig:sparsify_curve}
    \end{subfigure}
    \begin{subfigure}{0.495\textwidth}
        \resizebox{\linewidth}{!}{\input{figures/sparsify/error.tex}}
        \subcaption{Sparsification Error for all methods\label{fig:sparsify_error}}
    \end{subfigure}
    \caption{
        \textbf{Unimodal uncertainty quantification:} Sparsification results of analyzed methods with respect to the disparity BadPix007.
        By removing a certain fraction with the highest predicted uncertainty (a), the error decreases.
        The ``Oracle'' is a lower bound, created by removal of truly worst pixels.
        We also compute the difference between the predicted sparsification and its ``Oracle'', denoted as Sparsification Error (SE) (b), for a comparison of the three methods (trained on all depth modes)
    }
    \label{fig:sparsify}
    \vspace{-3mm}
\end{figure*}
Previous methods and datasets~\cite{honauer2016dataset} always consider the disparity of the closest object as ``true'', even when this object is transparent.
However, estimation methods oftentimes output the disparity of the background object in those cases, which may lead to severe issues in downstream applications.
In addition, more ambiguities usually occur in non-textured areas which cannot be estimated correctly.
Most optimization-based methods fill in those ambiguous regions by interpolation between adjacent pixels with confident predictions.
Due to the limited receptive field of neural network based methods, this is only possible to some extent.
In any case, a confidence measure is extremely useful for downstream applications in order to decide if an estimate can be trusted.
To achieve this, the overall variance $\sigma^2$ of the predicted posterior distribution can be used as an uncertainty measure.
We aim for a consistently high uncertainty in regions with ambiguous predictions.
To evaluate the quality of the estimated posteriors,
we remove the $s\%$ of pixels with the highest posterior variance (uncertainty).
With these ambiguous and uncertain cases filtered out, the BadPix of the remaining pixels is lower,
which can be plotted as a sparsification curve (see \cref{fig:sparsify_curve}).
The optimal curve can be computed by removing those $s\%$ of pixels with the largest ground truth error.
We call this the ``oracle'' curve, 
which represents the lower bound of what is achievable.
This method is commonly used to evaluate uncertainties for regression tasks~\cite{ilg2018uncertainty}.
In order to compare all methods, we compute the Sparsification Error (SE) by subtracting the oracle curve from the sparsification curve.
The Area under the Sparsification Error (AuSE) quantifies the uncertainty quality of each method with a single number.


\subsubsection{Multimodal Prediction}
\newcommand{\columnSpace}{3pt}
\addtolength{\tabcolsep}{\columnSpace}
\begin{table*}[h]
    \begin{center}
        %\newcolumntype{d}[1]{D{.}{.}{#1}}
        %\resizebox{\linewidth}{!}{
        \begin{tabular}{l|r r | r r r | r | r}
        \hline
            \textbf{Method} &
            \multicolumn{2}{c|}{\textbf{Unimodal Metrics}} &
            \multicolumn{3}{c|}{\textbf{KL Divergence}} &
            \textbf{AuSE} $\downarrow$&
            \textbf{Time} $\downarrow$\\
            &
            MSE $\downarrow$&
            BadPix $\downarrow$&
            Unimodal $\downarrow$&
            Multimodal $\downarrow$&
            Overall $\downarrow$&
            &  (in sec)    \\
        \hline
        \hline
            BASE (uni) &
            \textbf{0.374} & 0.229 & 4.720 & 7.876 & 5.421 & - & \textbf{2.188} \\

            BASE (multi)  &
            0.563 & 0.307 & 5.259 & 8.514 & 6.025 & - & 2.211 \\
        \hline
            UPR (uni) &
            0.439 & 0.235 & 1.719 & 3.381 & 1.879 & \textbf{0.071} & 2.260 \\

            UPR (multi) &
            0.676 & 0.285 & 1.987 & 3.156 & 2.114 & 0.072 & 2.287 \\
        \hline
            ESE (uni) &
            1.269 & 0.223 & 4.164 & 3.628 & 4.160 & 0.099 & 17.492 \\

            ESE (multi) &
            1.850 & 0.229 & 4.283 & 3.719 & 4.277 & 0.121 & 16.902 \\
        \hline
            DPP (uni) &
            0.765 & \textbf{0.209} & \textbf{1.631} & 3.057 & \textbf{1.734} & 0.272 & 4.348 \\

            DPP (multi) &
            0.686 & 0.231 & 1.824 & \textbf{2.987} & 1.914 & 0.197 & 4.382 \\
        \hline
        \end{tabular}
        %}
    \end{center}
    \vspace{-3mm}
    \caption{
        \textbf{Evaluation}, from left to right:
        Mean Squared Error and the common BadPix007 score (percentage of pixels with $|y_i - \hat{y}_i| > 0.07$),
        Kullback-Leibler divergence on unimodal, multimodal and all pixels,
        Area under Sparsification Error (AuSE),
        runtime of one forward pass.
        Our methods were trained with both losses $\mathcal{L}_x$ (uni) and $\mathcal{L}_x^{\mathrm{MM}}$ (multi) respectively.
        Lower is better
    }
    \label{tab:results}
\end{table*}
For many applications, including rerendering of a recorded scene from different angles, estimating multiple depths for pixels at object edges and transparent surfaces is desirable.
In addition to the disparities of all modes, the contribution of each mode to the color of the pixel is also important.
To evaluate both, we measure the Kullback-Leibler divergence (KLD) 
\begin{equation}
    \mathcal{D}_{\mathrm{KL}} = \int p(y_i) \log \left( \frac{p(y_i)}{p(y_i | x_i)} \right)
\end{equation}
between the predicted disparity posterior $p(y_i | x_i)$ and the true disparity distribution $p(y_i)$ at a pixel $i$.
Intuitively, the KLD will be minimal if the posterior assigns a high probability density to each true disparity mode and a low density to disparities that are not present at a pixel $i$.
In other words: the KLD is lowest, if each mode is recovered sharply, instead of a broad uncertainty covering both.
E.g.\ in~\cref{fig:teaser_posteriors}, the green and orange curves have the same uncertainty, but the green has a much lower KLD.
Optimally, the density at each disparity mode corresponds to the contribution $\eta_i$ of this mode to the resulting pixel color.
As the KLD is only well defined between two continuous or two discrete distributions and we compare continuous as well as discrete methods, we chose to discretize all distributions.
We therefore assign each ground truth disparity to one out of $K = 108$ bins with a width of $h \approx 0.065\mathrm{px}$ each.
\begin{equation}
    p(y_k) =  \sum_j p(y_j) \; \forall j \; \mathrm{with} \; | y_j - y_k | < \frac{h}{2}
\end{equation}
This is, again, motivated by the well-established BadPix007 metric~\cite{honauer2016dataset} which considers a pixel as correct if the $\mathcal{L}_1$ distance to the ground truth is below $0.07\mathrm{px}$.
For the baseline method that only outputs one disparity, we simply set the probability of the bin that contains this disparity to $1$.
All continuous posterior distributions are discretized by integrating over the interval of each bin:
\begin{equation}
    p(y_k | x) = \int\limits_{(k-0.5) h}^{(k+0.5) h} p(y | x) \mathrm{d}y
\end{equation}
We now average the discrete KLD
\begin{equation}
    \mathcal{D}_{\mathrm{KL}} = \frac{1}{NK} \sum\limits_{i} \sum\limits_{k} p(y_{ik}) \log \left( \frac{p(y_{ik})}{p(y_{ik} | x_i)} \right)
\end{equation}
over all pixels in all validation scenes.
In addition, we also compute the KLD over all unimodal and all multimodal pixels separately. 
A pixel is considered multimodal if it has at least two modes $j$ with $p(y_j) > 0.3$.




% At depth edges, the dataset ground truth only contains one disparity mode, although multiple modes are valid (compare \cref{fig:ground_truth}).
% We therefore select the two most likely disparities from the posterior distribution, but only evaluate the closest one to the ground truth.
% Although DPP, ESE and IB-INN are able to predict a large number of modes, we limited the evaluation to bimodal cases
% because only two valid disparities exist for the vast majority of multimodal pixels.
% A selection of the best mode gives us a lower bound for our error metrics in multimodal areas, denoted as MSE-LB and BadPix-LB.

\subsubsection{Results}
% \begin{figure*}[t]
%     \centering
%     \begin{subfigure}{0.195\textwidth}
%         \includegraphics[width=\textwidth, trim= 0 0 0 0, clip]{figures/dummy}
%         \subcaption{Center View}
%     \end{subfigure}
%     \begin{subfigure}{0.195\textwidth}
%         \includegraphics[width=\textwidth, trim= 0 0 0 0, clip]{figures/dummy}
%         \subcaption{First disparity (ESE)}
%     \end{subfigure}
%     \begin{subfigure}{0.195\textwidth}
%         \includegraphics[width=\textwidth, trim= 0 0 0 0, clip]{figures/dummy}
%         \subcaption{Second disparity (ESE)}
%     \end{subfigure}
%     \begin{subfigure}{0.195\textwidth}
%         \includegraphics[width=\textwidth, trim= 0 0 0 0, clip]{figures/dummy}
%         \subcaption{First disparity (DPP)}
%     \end{subfigure}
%     \begin{subfigure}{0.195\textwidth}
%         \includegraphics[width=\textwidth, trim= 0 0 0 0, clip]{figures/dummy}
%         \subcaption{Second disparity (DPP)}
%     \end{subfigure}
%     \caption {
%         \textbf{Multimodal depth estimation results.} For an exemplary scene from our dataset (a), we visualize the first and second disparity mode as estimated by ESE (b, c) and DPP (d, e)
%         \label{fig:qualitative_results}}
% \end{figure*}
% undo what i did beofre the table (+5pt)
\Cref{tab:results} compares the unimodal, multimodal and sparsification performance of all methods.
In the following, we will interpret our results with respect to the aforementioned applications: unimodal disparity estimation with uncertainty and multimodal disparity estimation.

With respect to pure unimodal performance, our baseline method and DPP perform best.
The higher MSE for DPP is caused by small discretization errors due to the discrete number of bins.
Those small errors are well below a threshold of $0.07\mathrm{px}$ and therefore ignored by the BadPix metric
which shows that DPP indeed predicts $2\%$ more pixels correctly compared to the baseline.
UPR performs only slightly worse than both methods overall.
However, due to the uncertainty being directly supervised by $\mathcal{L}_{\mathrm{UPR}}$ this method is superior in terms of sparsification.
This means that its uncertainty metric reflects most accurately whether a prediction is correct.
We conclude that, if the application requires only a single disparity and confidence is important, UPR should be considered.

With respect to the accuracy of the predicted posterior distribution, DPP performs best in unimodal and also multimodal areas.
However, as most softmax prediction methods, it is overconfident, as reflected by the sparsification error in~\cref{fig:sparsify_error}.
Despite the popularity of ensemble-based models for uncertainty estimation, ESE cannot compete with the other two methods.
It especially performs worse in highly non-textured areas with a large and noisy uncertainty output $b_i$ for all ``ensemble members''.
To decide for a unimodal disparity estimate, the member with the lowest uncertainty is still used, but due to the noise, this choice becomes arbitrary.
The chosen member can only output a disparity from a small interval within the potentially large disparity range. 
On average, this causes a high deviation from the ground truth for ESE.
In contrast, our other methods are able to ``smooth'' the disparity in uncertain areas from adjacent, more certain pixels.
This is also reflected by the relatively high MSE but low BadPix error:
the amount of ``correctly'' predicted pixels is on par with other methods, but the deviation of ``wrongly'' predicted pixels is generally higher.
In addition, as all members contribute slightly to the mixture of Laplacians, the density of the posterior is higher along the whole disparity interval, which leads to a worse multimodal KLD compared to UPR and DPP.
We therefore generally recommend DPP for multimodal predictions in small, narrow-baseline light fields.
However, due to its shift-operation, ESE can, unlike other methods, operate on arbitrary large disparity ranges and is therefore still advisable for high-resolution or wide-baseline light field cameras.
In addition, it performs also relatively well in terms of sparsification.
Comparing the methods trained on only one mode with the same methods trained on multiple modes shows that multimodal training leads to a slightly better multimodal performance for UPR and DPP, but always comes at a cost in unimodal areas.
Our baseline method cannot efficiently represent multimodal posteriors as it only predicts a single disparity.

We conclude that the exact model and training method should be carefully chosen based on the intended application.
We refer to~\cref{sec:additional_experiments} for examples of estimated disparity posterior distributions, an evaluation of our methods on the common HCI 4D Light Field Dataset~\cite{honauer2016dataset}, additional qualitative results as well as a comparison to Sinha \etal~\cite{sinha2012image} and Johannsen \etal~\cite{johannsen2016sparse}.



%In general, it can be seen, that the unimodal predictions provided by UPR tend to perform best if the unimodal assumption holds.
%The overall results are on par with the state-of-the-art method EPI-Net.
%As one might expect, ESE improves the performance in multimodal areas, by extending UPR to a multimodal posterior.
%Due to its ensamble nature it has a much longer runtime.
%However, one should bare in mind that only the EPE method can handle large disparities, which might be relevant for some applications.
%The results for DPP clearly indicate that discritization improves multimodal estimation by a big margin.
%Additionally, it delivers a superior sparsification quality.
%Nevertheless, due to its generative nature, the IB-INN yields to the most accurate posterior prediction, which is clearly indicated by the multimodal and even unimodal performance.
%Because the INN architecture has the lowest number of parameters, it is also the fastest method.
%It also yields the lowest Bimodality Error, which makes it suitable to classify unimodal and multimodal pixels (bimap prediction).
%The overall MSE indicates that discritization still comes at a cost.
%However, one could avoid this by using the predicted bimap to join unimodal predictions from \eg UPR with bimodal predictions from the IB-INN.
% UPR is the only method in our comparison that assumes a single valid disparity mode.
% Thus, it clearly performs best if this assumption holds.
% As one might expect, its overall results are on par with the state-of-the-art method EPI-Net.
% From the high AuSE of UPR, we conclude that modeling multiple modes also improves the uncertainty estimation performance.
% ESE extends UPR to multiple modes and therefore, as expected, improves the performance in multimodal areas.
% Although this comes at the cost of an extended runtime and worse overall performance, one should bare in mind that ESE is the only method which can handle large disparities relevant for many applications.
% One key observation is that the discrete methods, namely DPP and IB-INN, are superior for multimodal depth estimation.
% Especially the IB-INN outperforms all other methods w.r.t.\ multimodal MSE, BadPix and AuBE.
% Those improvements come at nearly no cost as the overall depth accuracy is on par with state-of-the art methods and the runtime is even lower.
% Only the overall MSE increased slightly which is most likely caused by the discretization.
% We argue that these improvements are not only caused by the formulation as a discrete classification problem, but rather are a consequence of the generative nature of the IB-INN.
% This becomes obvious when comparing its results to the na\"ive DPP model.
% Surprisingly, DPP has a much lower AuSE.
% However, higher estimation accuracy usually makes uncertainty quantification more difficult and might therefore explain this gap.
%\Cref{fig:qualitative_results} shows a qualitative result of the IB-INN for a semi-transparent object.

==> Towards Multimodal Depth Estimation from Light Fields/sections/introduction.tex <==
%TEX root = ../paper.tex
\begin{figure}[h]
    \centering
    \begin{subfigure}{0.495\textwidth}
        \centering
        \includegraphics[width=0.495\textwidth]{figures/teaser/main}
        \includegraphics[width=0.495\textwidth]{figures/teaser/layers}
        \subcaption{Rendered scene (left) containing multiple disparity layers (right)}
        \vspace{0.3cm}
    \end{subfigure}
    \begin{subfigure}{0.495\textwidth}
        \resizebox{\linewidth}{!}{\input{figures/teaser/teaser.tex}}
        \subcaption{\label{fig:teaser_posteriors}Disparity posterior distributions, predicted by different methods}
    \end{subfigure}
    \caption{
        \textbf{Comparison of disparity posterior distributions}. 
        Synthetic scene (a) containing overlapping objects at different depths.
        (b) shows disparity posterior distributions, estimated by different methods, for a single pixel (red crosses in (a)).
        This pixel captured two disparity modes (mesh material of chair (foreground) and wooden wall (background)).
        Note, that the Unimodal Posterior Regression (UPR) network, which outputs the mean and width of a Laplacian distribution, makes a wrong and uncertain prediction.
        The EPI-Shift Ensamble (ESE) detects both valid modes near the ground truth (GT).
    }
    \label{fig:teaser}
    \vspace{-3mm}
\end{figure}
Light field recordings and their applications, like real time rendering for virtual reality or highly accurate depth estimation, have improved vastly in recent years.
However, while light field rendering methods handle transparent and reflective objects well, current depth estimation methods still perform poorly in those areas.
% Nevertheless, the exact depth of objects in the scene is still desirable, \eg to add objects or edit the scene before rendering.
State-of-the-art depth estimation methods mainly fail in three corner cases:
at objects edges, semi-transparent and reflective surfaces.
All three are caused by multiple objects at different depths contributing to the projected color of a single pixel on the camera sensor.
Most existing models fundamentally ignore these cases and assume only one ``true'' depth for each pixel.

% The contribution of colors to a pixel is influenced by countless effects in the imaging process: the spread of an infinitesimally small point to a finite area on the image sensor modeled by its point spread function (PSF)~\cite{Kerviche2017}, reflection, refraction and diffraction of light, depth of field, motion blur, and the Bokeh effect, to just name a few.
% Modeling these effects explicitly is a complex endeavour, especially when all types of cameras should be covered.

Instead, we propose a series of deep-learning based methods to perform multimodal depth estimation, and depth estimation with uncertainty estimates.
For this, we start with the basic idea of outputting Bayesian posteriors, whereas standard regression models just produce a single estimate. 
From this idea, and by using a simple and well-founded maximum likelihood training framework, we develop three different light field depth estimation methods, all three of which are able to infer uncertainty estimates, and use multiple ground truth values during training. 
Two of the proposed methods are also able to predict multiple distinct depth values per pixel at test time.

To train our methods, we propose to utilize a multimodal dataset that contains the exact depth, color and opacity of all depth planes that are visible in an image. 
This is, in contrast to other current datasets which only contain a single ``true'' depth value.
Our multimodal dataset consists of randomly generated synthetic scenes with a significant proportion of occlusion and transparent objects.
This, for the first time, enables supervised training of multimodal depth estimation.

\hfill \newline
Our main contributions are as follows:
\begin{itemize}
\item 
An exploration of our three novel deep learning methods for light field based depth estimation being able to handle multiple depth modes:
\emph{(i)} Unimodal Posterior Regression (UPR); \emph{(ii)} EPI-Shift-Ensemble (ESE); \emph{(iii)} Discrete Posterior Prediction (DPP)
\item The release of the first multimodal light field dataset, containing the depth of all objects and their contribution to the color of each pixel in an image
\item A thorough evaluation of the predicted depth posterior distributions. We observe that the more restrictive UPR method works well when the unimodal depth assumption of traditional methods holds. In cases where it does not, the model is able to express a high uncertainty. In general, the discrete DPP method is superior to UPR and ESE.
\end{itemize}

==> Towards Multimodal Depth Estimation from Light Fields/sections/method.tex <==
% !TEX root = ../paper.tex
\newcommand{\shift}{\mathit{shift}}
%In this section, we describe the methods, we evaluated in detail.
%We first motivate and describe the basic idea of depth estimation from light fields.
%Secondly, we describe our extensions to four uncertainty estimation for regression tasks, three of which can be used to infer multiple modes.
%Third, the utilized network architectures are explained in detail.
%\todoLA{just cut the whole spiel about different depth estimation apporaches?}
%In general, there are different image input modalities that can be used for depth estimation.
%The least informative input is a single RGB image. 
%Of course, depth estimation in this case is a highly ill-posed task and largely relies on high-level semantic information.
%This results in huge uncertainties, that do not contain the type of measurable ambiguities and multi-modalities we are interested in.
%A step up from this, stereo image pairs give more constraints.
%But still, the task is ill-defined \eg at occlusion edges, where objects are only visible in one of the images.
%Instead, the most accurate depth estimation from images is possible using light fields, which contain the fewest ill-defined cases. 
%This makes light fields the most interesting candidate for accurately identifying multi-modal or ambiguous cases when they arise.
%
% \begin{figure}[t]
%     \centering
%     \begin{subfigure}{0.224\linewidth}
%         \includegraphics[width=\textwidth]{figures/epi_extraction/epi_extraction_a.png}
%         \subcaption{
%             Light field
%         }
%     \end{subfigure}
%     \begin{subfigure}{0.3\linewidth}
%         \includegraphics[width=\textwidth]{figures/epi_extraction/epi_extraction_b.png}
%         \subcaption{
%             Vertical stack
%         }
%     \end{subfigure}
%     \begin{subfigure}{0.44\linewidth}
%         \includegraphics[width=\textwidth]{figures/epi_extraction/epi_extraction_c.png}
%         \subcaption{
%             EPI Extraction
%         }
%     \end{subfigure}
%     \caption{
%         Extraction of an \textbf{Epipolar Plane Image (EPI)}.
%         One exemplary column from all view points (a) is selected and stacked (b).
%         An EPI is extracted, by slicing along one view dimension (c).
%         Note the diverse slopes of lines in the EPI which are equal to the negative inverse disparities
%     }
%     \label{fig:epi_extraction}
%     \vspace{-3mm}
% \end{figure}
Before we introduce our posterior estimation methods, we explain the basics of light field depth estimation.
A 4D light field is typically recorded by a 2D array of cameras, aligned on a regular grid.
Each camera is assigned a pair of so-called view coordinates $(u, v)$, \eg $(1, 1)$ for the top left camera.
Each pixel in an image is then also assigned a pair of image coordinates $(s, t)$.
A slice along one axis in image space with the corresponding axis in view space, \eg fixing $u$ and $s$, forms a so-called Epipolar Plane Image (EPI).
Each pixel in the central camera view is visible as a line structure in the EPI.
The slope of this line is equal to the negative inverse disparity of the pixel.
Thus, the task of depth estimation from light fields is to robustly detect this slope.
%However, algorithms often face problems in challenging and ambiguous cases: 
%non-textured regions, specular reflections, depth edges and semi-transparent regions.
%In this work we make progress for these cases by estimating the full depth posterior.
%In particular the last two cases involve not a single but multiple valid depths.
%In contrast to previous work we find those multimodal ambiguities.
However, this approach assumes opaque, smooth and lambertian surfaces.
Non-textured, specular or semi-transparent regions and depth edges are ambiguous and therefore challenging even for state-of-the-art methods.
In this work we make progress for these cases by estimating the full depth posterior distribution.
This is especially useful for pixels with more than one valid depth mode, caused by either semi-transparency or the point spread at depth edges.
Unlike previous works that only predict a single depth, we are able to find those modes.

%For the last two cases, there are multiple distinct and equally valid disparities for each pixel,
%\eg for the transparent foreground object and the background.
%However, these multimodal ambiguities have so far not been addressed explicitly in previous work.
%Therefore, this paper aims to analyze such cases by full posterior estimation methods.


%We argue that in order to make progress for these cases, it is necessary to estimate the depth posterior distribution.
%In particular latter two challenges (semi-transparency and depth edges) involve not a single but multiple valid depth modes per pixel.
%In contrast to previous work, we model full posterior distributions, which are able to capture multiple modes with their respective uncertainty. 
%The focus of our work is to extend and evaluate four different posterior estimation methods.

\subsection{Posterior Estimation}\label{sec:uncertainty}
From here on, we will simply refer to the input of a depth estimation network as $x$,
and to disparity as $y$.
In practice, the input to a depth estimation network is a concatenation of horizontal, vertical and diagonal EPIs.
Standard regression models usually output a single guess for the disparity, $\hat y = f_w(x)$,
where $f_w$ could be EPI-Net~\cite{shin2018epinet} with network weights denoted as $w$.
Instead, our goal is to estimate the posterior distribution $p(y\mid x)$ of the disparity $y$ given an input light field $x$.
In the following, we present four different approaches that all model such a posterior distribution.

To supervise more complex posterior distributions that can represent more than one mode, we created our own multimodal depth dataset.
Unlike common datasets that only contain a single ground truth disparity $y_i$ for each pixel $i$, we include the
disparities of multiple depth modes $y_{ij}$ for transparent objects and depth edges.
For each disparity we also include the amount of color $\eta_{ij}$ that it contributed to the pixel, 
\ie the perceived opacity of that object in the pixel.
From a Bayesian perspective, we interpret $\eta_{ij}$ as the probability $p(y_{ij})$ of this disparity.
This choice is justified in both an intuitive and methodological sense:
$\eta_{ij}$ corresponds to the fraction of the pixel's area that is taken up by the object at depth $y_{ij}$.
Lacking any prior knowledge, this is also equal to the probability that the depth at any subpixel position corresponds to that object.
This equality between the opacity $\eta_{ij}$ and probability $p(y_{ij})$ 
is valid both at edges as well as fine structures such as grids or woven meshes.
We also extend the definition to apply to semi-transparent materials such as printed glass as a simplifying assumption.
In Appendix \ref{sec:opacity_probability}, we give a more rigorous examination of the connection between $\eta_{ij}$ and $p(y_{ij})$.



%Our aim is to find the posterior distribution $p(y | x)$ of the disparity $y$ given an input light field $x$.
%We compare four deep-learning based approaches to extract this distribution.
%We denote the standard approach EPI-Net \cite{}, as $f_w(x)=y$, with network parameters $w$. Note that traditionally this method only infers a single prediction,
%However, the disparity output $y$ could also be interpreted as mean $\mu$ of the posterior distribution $p(y | x)$.

\subsubsection{Unimodal Posterior Regression}
The most common approach for learning distributions is Maximum-Likelihood (ML) learning,
which most loss functions can be reformulated as.
The ML objective aims to find the model parameters $w$ which maximize the log likelihood of the training data 
$\{ (x_i, y_i) \}_{i=0}^N$ under the estimated posterior distribution.
In practice, we {minimize} the \emph{negative} log likelihood instead:
\begin{equation}
  \mathcal{L}_{\mathit{\mathrm{ML}}}  = - \frac{1}{N} \sum\limits_{i} \log p( y_i \mid x_i, w).
\end{equation}
It can be shown that this objective minimizes the Kullback-Leibler divergence (KLD) between $p( y \mid x, w)$
and the true posterior $p^*(y \mid x)$.

Previous regression based approaches \cite{shin2018epinet} simply use the $\mathcal{L}_1$ loss to make a single prediction:
\begin{equation}
  \mathcal{L}_{1}  = \frac{1}{N} \sum\limits_{i} | y_i - f_w(x_i) | .
\end{equation}
We see that this is equal to the ML objective when the posterior is assumed to be a Laplace distribution 
$p(y \mid x, w) \propto \exp( - | y - \mu | / b) / 2b$ with the network output $\mu = f_w(x)$ and a fixed value of $b=1$.
This motivates the following simple extension, 
which is an adaptation of the Dawid-Sebastiani-score \cite{dawid1999coherent}, later popularized in \cite{kendall2017uncertainties},
%where an $\mathcal{L}_2$-loss and Gaussian posterior are used instead:
except that the $\mathcal{L}_2$-loss corresponding to a Gaussian posterior was used instead:
we allow the network to change the width $b$ of the posterior. With this, it becomes 
\begin{equation}
p(y \mid x, w) = \frac{1}{2b} \exp\left( - \frac{| y - \mu|}{b}\right), \; \text{with} \quad [b,\mu] = f_w(x).
\end{equation}
Putting this back into the ML objective, we get the following loss function for the predictive uncertainty:
\begin{equation}
    \mathcal{L}_{\mathrm{UPR}} = \frac{1}{N} \sum\limits_{i} \frac{|\mu_i-{y}_i|}{b_i} + \log b_i,
    \; \text{with} \quad [\mu_i, b_i] = f_w(x_i).
    \label{eq:loss_upr}
\end{equation}

%A simple extension to the traditional, aiming for a posterior distribution instead of a single value, is to predict not only the mean $\mu$ but also the variance $\sigma^2$ of this distribution we denote as $\theta(x, w)$.
%To train this network, the log-likelihood of the training dataset
%\begin{equation}
%    \log p(D | w) = \frac{1}{N} \sum\limits_{i} \log p\left(y_i | \theta(x_i, w)\right)
%\end{equation}
%is maximized w.r.t this distribution \textbf{(TODO: motivate this)}.
%Usually, $\theta$ is modeled as a normal distribution, leading to an $\mathcal{L}^2$ loss with learned loss attenuation~\cite{Kendall2017}.
%However, previous works~\cite{Shin2018} show that the $\mathcal{L}^1$ loss performs better for regression tasks.
%We therefore chose to model the posterior with a Laplace distribution.
%The predictive uncertainty network $f_w(x) = (\mu, b)$ outputs the mean $\mu$ and diversity $b$ of this distribution.
%\begin{equation}
%    \log p(D | w) = \frac{1}{N} \sum\limits_{i} \log \left(\frac{1}{2b_i}\exp\left(-\frac{|\mu_i-y_i|}{b_i}\right)\right)
%\end{equation}
%which can be rewritten as
%\begin{equation}
%    \log p(D | w) = \frac{1}{N} \sum\limits_{i} -\log 2b_i -\frac{|\mu_i-y_i|}{b_i}
%\end{equation}
%In order to maximize this data likelihood, we minimize the predictive loss
%\begin{equation}
%    \mathcal{L}_{\mathit{pred}} = \frac{1}{N} \sum\limits_{i} \frac{|\mu_i-\hat{y}_i|}{b_i} + \log b_i
%    \label{eq:loss_pred}
%\end{equation}
%with $\hat{y}$ being the ground truth disparity for pixel $i$.
This loss can be understood intuitively:
If the network struggles to predict $y_i$, the $\mathcal{L}_1$ loss term can 
be down-weighted by increasing the scale parameter $b$ for this pixel.
To avoid the trivial solution $b_i\to \infty$ for any input, high $b$ are penalized by a regularization term $\log b$.
In practice, we let the network predict $\log b$ instead of $b$ to improve numerical stability.

This approach gives us a measure of aleatoric uncertainty~\cite{kendall2017uncertainties} for each pixel which is already helpful for many downstream applications.
However, the implicit assumption for the method to work well is that the true posterior is also Laplacian.
Needless to say, this is certainly not true in multi-modal cases, which cannot be modeled by the Laplace distribution.
%Nevertheless could multiple depth modes (as in our dataset) be useful to supervise to supervise this uncertainty.
With multiple ground-truth depth modes $y_{ij}$ as opposed to only $y_i$, as in our dataset,
the loss for a Laplace distribution becomes 
%In that case, the negative log likelihood for a Laplace distribution becomes
\begin{equation}
    \mathcal{L}_{\mathrm{UPR}}^{\mathrm{MM}} = \frac{1}{N} \sum\limits_{i} \sum\limits_{j} p(y_{ij}) \frac{| y_{ij} - f_w(x_i) |}{\log b_i} + \log b_i
\end{equation}
and can be applied to the $\mathcal{L}_1$ loss respectively:
\begin{equation}
    \mathcal{L}_{1}^{\mathrm{MM}} = \frac{1}{N} \sum\limits_{i} \sum\limits_{j} p(y_{ij}) | y_{ij} - f_w(x_i) |
\end{equation}
However, in any case, those networks will focus on a single mode, or lie in between, and compensate for its wrong prediction
by expressing a very high uncertainty like in~\cref{fig:teaser}.

\subsubsection{EPI-Shift-Ensemble}
Commonly, one way to circumvent this exact issue is to use an ensemble of networks.
Instead of just estimating a single posterior, $M$ networks predict $M$ different posteriors, which are then averaged:
\begin{equation}
    p(y | x ) = \frac{1}{M}\sum\limits_k p(y | x, w_k)
    \label{eq:monte_carlo}
\end{equation}
over all networks with learned weights $w_k$, $k=1\dots M$.
It has been shown that ensembles deliver some of the best uncertainty estimates among existing methods \cite{ovadia2019can}.
Their main limitation is the high computational cost, especially for training.
Various approaches try to avoid this and train only a single model. 
For instance, Monte Carlo dropout exhibits similar characteristics as a true ensemble \cite{hara2016analysis}.
Instead, we propose a new scheme which uniquely exploits the nature of light field data, which we term EPI-Shift-Ensemble (ESE).
To motivate this, we take note of the technique from \cite{leistner2019learning}, 
where the EPI is sheared in such a way that a global offset $\Delta y$ is added to the disparity of the EPI.
This is advantageous, because it enables inference on large disparities \eg for wide-baseline light field cameras.
We denote this operation as $\shift(x, \Delta y)$ and extend it to arbitrary sub-pixel steps. 
To form our EPI-Shift-Ensemble, we successively shift the input $M$ times in steps of $\Delta y$.
This gives us $M$ different augmented inputs, where each has a different artificial disparity offset.
Each input is fed into the network, and the resulting posteriors are shifted back by the same offset.
In this way, we get $M$ different estimates by the same network, each from a different input containing the same information.
The overall posterior can be expressed as
\begin{equation}
    p_\mathit{ESE}(y \mid x, w ) = \frac{1}{M}\sum\limits_{k}
    p\Big(y - k\cdot \Delta y \Big| \shift(x, k \cdot \Delta y) , w\Big).
\end{equation}
In the summation, $k= -\lfloor M/2 \rfloor \dots \lceil M/2 \rceil$. 
For the shape of the individual posteriors, we use the same Laplacian as before.
Note that the network weights $w$ are shared for each summand, only the shift is different.
%To circumvent this, we extend the predictive uncertainty network based on the idea of Bayesian deep learning.
%From a Bayesian view point, in order to model an arbitrary posterior distribution, one could marginalize
%\begin{equation}
%    p(y | x, D) = \int p(y | x, w) p(w | D) \mathit{d}w
%    = \int p(y | \theta(x, w)) p(w | D) \mathit{d}w
%\end{equation}
%over the distribution of all network parameters $w$, given the dataset $D$.
%Of course, this integral cannot be computed efficiently in practice.
%Instead, common methods make use of Monte Carlo integration by sampling a discrete number of networks from $w_i \sim p(w|D)$.
%This can be done with Monte Carlo dropout, which is performed by $M$ forward passes for inference with dropout applied~\cite{Gal2016}.
%Alternatively, an ensemble of $M$ networks with different random initialization is trained~\cite{Ilg2018}\cite{Kendall2017}.
%Using those samples, the posterior distribution
%\begin{equation}
%    p(y | \theta(x, w)) \approx \frac{1}{M}\sum\limits_i p(y | \theta(x, w_i))
%    \label{eq:monte_carlo}
%\end{equation}
%can be approximated by using Monte Carlo integration.
%Usually, Bayesian deep learning techniques are used to also capture model uncertainty arising from a lack of training data.
%However, recent deep learning based light field depth estimation techniques are trained solely using synthetic data, which can be generated cheaply.
%Instead, we are only interested in a more expressive model for our posterior distribution.
%We therefore fix the network parameters $w$ and sample from the input distribution $x_i \sim p(x|D)$ instead with $p(x|D)$ being a uniform distribution over the interval of disparities that are present in our dataset $D$.
%Thus, our Monte Carlo integration changes to
%\begin{equation}
%    p(y | \theta(x, w)) \approx \frac{1}{M}\sum\limits_i p(y | \theta(x_i, w))
%\end{equation}
%For the sampling process from $p(x|D)$ we chose borrow the idea of EPI-Shift from~\cite{Leistner2018} which efficiently lets us add a constant disparity offset to the whole input light field $x$.
However, this operation alone does not prevent the problems seen for the single mode approach:
the network will try to average out bi-modal solutions, or collapse into one mode.
As a result, we see little to no diversity in the EPI-Shift-Ensemble, and no multi-modal posteriors.
To prevent the collapse, we mask the loss during training so that it only applies to pixels with a shifted $y' = y - k \cdot \Delta y$ within the range of one step $|y'| < \Delta y / 2$.
In all other cases the output will have a large uncertainty:
\begin{equation}
\mathcal{L}_{\mathrm{ESE}} = 
    \frac{1}{N}\sum\limits_{i}
    \begin{cases} 
        \frac{|\mu_i-{y}_i|}{b_i} + \log b_i & \text{if } |{y_i'}| < \frac{\Delta y}{2} \\
        0 & \text{otherwise.}
    \end{cases}
    \label{eq:loss_ese}
\end{equation}
We extend this to our multimodal dataset similarly to our unimodal networks:
\begin{equation}
\mathcal{L}_{\mathrm{ESE}}^\mathrm{MM} = 
    \!\frac{1}{N}\! \sum\limits_{i}\sum\limits_{j}
    p(y_{ij})
    \begin{cases} 
        \frac{|\mu_{i}-{y}_{ij}|}{b_{i}} \!+\! \log b_{i} \!\! & \!\! \text{if } |{y_{ij}'}| < \frac{\Delta y}{2} \\
        0 & \text{otherwise.}
    \end{cases}
    \label{eq:loss_ese_mm}
\end{equation}
After training with this loss, the network will only be confident (narrow posterior) if 
it estimates that the input disparity is $y \in [-\Delta y / 2, \Delta y / 2]$,
and the predicted posterior will always be centered in this range.
When using this network in the EPI-Shift-Ensemble, 
we see that each term $k$ will only contribute a narrow posterior if a plausible disparity
lies between $(k - 1/2) \Delta y$ and $(k + 1/2) \Delta y$, 
thus ensuring diverse outputs and the possibility of multi-modal predictions.
% Compared to~\cite{Leistner2019}, we do not need an additional classification loss to select the most confident prediction.
Three details should be noted:
First, the model is not trained as an ensemble, a single model is trained just as before with the modified $\mathcal{L}_\mathrm{ESE}$-loss.
The ensembling operation is only performed at inference time.
Second, the masked loss does not reduce the effective size of our training set, as we also apply random EPI-shifts as a part of the data augmentation process.
This way, all pixels will randomly fulfill $|{y_i}| < \Delta y / 2$ at some point.
Lastly, the inference time is $M$ times longer, as $M$ forward passes have to be performed to compute the EPI-Shift-Ensemble.

\subsubsection{Discrete Posterior Prediction}
The approach of discretizing regression tasks has been successful for stereo depth estimation in the past,
and promises to model more expressive posteriors.
Specifically,
by discretizing the range of disparities, a softmax output can be used to represent the posterior.
The posterior is then a step function consisting of these discrete probabilities.
If $y_j$ are the discretization steps, we can write
\begin{equation}
    % p(y|x) \propto \mathit{softmax}\left(f_w(x_i)\right) = 
    % \frac{\exp\left(\sum\limits_j f_w(x_i)_j * p(y_{ij})\right)}
    % {\sum\limits_j \exp\left(f_w(x_i)_j\right)}
    p(y_j|x) \propto \mathit{softmax}\left(f_w(x_i)\right)_j \coloneqq
    \frac{\exp\left( f_w(x_i)_j \right)}
    {\sum\limits_k \exp\left(f_w(x_i)_k\right)}
\end{equation}
If multiple modes are used for the training, we also discretize the distribution $p(y_j)$ over these modes.
% \begin{equation}
%     \quad J(y) = \mathit{argmin}_j | y - y^{(j)} |.
% \end{equation}
Maximum likelihood training is then simply equivalent to the categorical cross-entropy (CE) loss,
where the correct ``class'' is the bin $j$ that the training example $y_i$ lands in:
\begin{equation}
    \mathcal{L}_{\mathrm{CE}} = \frac{1}{N} \sum_i
    - \log \Big(
    \mathit{softmax}\big(f_w(x_i)\big)_j \Big).
    \label{eq:loss_ce}
\end{equation}
For the multimodal dataset, we can compute the cross-entropy accordingly:
\begin{equation}
    \mathcal{L}_{\mathrm{CE}}^{\mathrm{MM}} = \frac{1}{N} \sum_i \sum_j
    - p(y_j) \log \Big(
    \mathit{softmax}\big(f_w(x_i)\big)_j \Big).
\end{equation}
Note, that the two correspond, for a unimodal dataset, we simply have $p(y_j) = 1$ and $p(y_{l \neq j}) = 0$,
simplifying to the cross-entropy in Eq. \ref{eq:loss_ce}.

Although the discrete posterior prediction gives us an uncertainty estimation at much lower computational cost than the EPI-Shift-Ensemble 
and can represent more flexible posteriors compared to simple Laplacians,
softmax probabilities are generally known to be overconfident \cite{guo2017calibration}
and also make wrong but confident predictions in ambiguous or unseen cases.
Different techniques for post-calibration of uncertainties exist, outlined in \cite{guo2017calibration}.
However, while they may prevent overconfidence going from the training to a test set, 
they do not make the uncertainties more reliable in general \cite{ovadia2019can},
\eg for ambiguous inputs.

%As an alternative, we could simply sacrifice some accuracy and discretize the disparity output into $M$ discrete labels.
%Therefore, we train our network to output a vector of scores for each label.
%We get an approximate posterior distribution
%\begin{equation}
%    p(y|x) = \mathit{softmax}\left(f_w(x)_y\right).
%\end{equation}
%by normalizing this vector with softmax.
%This enables us to detect multiple modes, if the modes are further apart than the disparity distance between adjacent labels.
%In addition, if we choose only one mode $\mu$, we can compute the variance
%\begin{equation}
%    \sigma^2 = \sum\limits_y (\mu - y)^2 p(y|x)
%\end{equation}
%which can be used as an uncertainty measure.
%Similar to most classification tasks we maximize the posterior entry for the true class, using the cross-entropy loss
%\begin{equation}
%    \mathcal{L}_{\mathit{CE}} =
%    -f_w(x)_{\hat{y}}
%    \log \left(
%        \sum\limits_y \exp\left(f_w(x)_y\right)       
%    \right)
%    \label{eq:loss_ce}
%\end{equation}
%with $\hat{y}$ being the ground truth label and $f_w(x)_y$ being the entry for class $y$ in the score vector.
%Although, this method gives us an uncertainty estimation at much lower computational cost, it is known to be poorly calibrated \textbf{(Weinberger paper)} and therefore delivers an inaccurate uncertainty measure.
%
%\subsubsection{Information Bottleneck INN}
%In machine learning research, 
%there has been a long standing alternative to standard softmax classifiers (termed discriminative classifiers or DCs in this context). 
%This alternative are so-called generative classifiers (GCs), \eg~\cite{Rubinstein1997}.
%They do not suffer as much from the weaknesses seen in DC outputs \cite{Ng2002}.
%In short, GCs don't estimate the posterior at all, 
%instead they model the conditional data distribution $p(x|y)$.
%The posterior is then obtained through Bayes rule.
%While this is difficult for the continuous case, the discrete posterior case is straight forward:
%\begin{equation}
%    p(y^{(j)} | x) = \frac{p(x | y^{(j)}) p(y^{(j)})}{\sum_{k}p(x|y^{(k)})p(y^{(k)})}.
%\end{equation}
%The relevant advantages of training such a GC instead of a DC for our application 
%are the better generalization, robustness and that the posterior obtained through Bayes rule is more accurate.
%While different approaches for training GCs have existed in the past, 
%\cite{Ardizzone2020} recently proposed a method that trains them efficiently and also delivers good performance.
%Their method applies the so-called Information Bottleneck (IB) objective from information theory as a training loss $\mathcal{L}_{\mathit{IB}}$,
%which models the trade-off between task performance and generative capabilities explicitly through a hyperparameter $\beta$.
%The resulting model is an invertible neural network $g_w$ (hence the name IB-INN), 
%that models the likelihood in a similar way to normalizing flows:
%The INN maps the input $x$ to a latent space $z$, with a prescribed conditional distribution $p(z|y)$.
%Each $p(z|y)$ is a standard normal distribution with a learned mean, so that $p(z)$ is a Gaussian mixture model (GMM).
%The density of the input is then parametrized using the change-of-variables formula:
%\begin{equation}
%    p(x \mid y) = p(z = g_w(x) \mid y) \left| \det\left(  \frac{\partial g_w(x)}{\partial x} \right) \right|.
%\end{equation}
%The main reason for using the INN architecture is that the Jacobian determinant $\det(  \partial g_w / \partial x )$
%can be efficiently computed, in contrast to standard feed-forward networks.
%Because we want to make a pixel-wise prediction, and not just a single class, 
%we have to slightly adapt the method used in \cite{Ardizzone2020}, and modify the latent space.
%Namely, we partition the latent space into subspaces, so that each subspace corresponds to one input pixel.
%Each subspace has its own GMM, but the parameters of the Gaussians are shared across subspaces,
%to that the GMM in each pixel looks the same.
%This extension allows the IB-INN to be fully convolutional and make a pixel-wise prediction.
%Details and a formal description can be found in~\cref{sec:architectures}.
% Formally, if we index each pixel subspace with $[l]$ ($l$: pixel number $1\dots W$.), 
% we write the conditional latent distribution as factorized:
% \begin{equation}
%     p(z_{[1:W]} | y_{[1:W]}) = \prod_l p_\mathit{Pix}(z_{[l]} | y_{[l]})
% \end{equation}

%- there is a latent space and it works though change of variables

%-it is a gaussian mixture 

%- the addition to \cite{Ardizzone2020}: we factorize the latent space over pixels
%\begin{equation}
%    p(z | y) = \prod_{\text{Pixels } l} p(z_l | y_l)
%\end{equation}

%- there is a GMM per pixel, but the mixtures are all the same

%- bing bang, it works the same as the discretization approach, but the results are better

%
%Alternatively, we also evaluate a method proposed by~\cite{Ardizzone2020}.
%An Invertible Neural Network (INN) is used to transform an input light field $x$ into a per-pixel latent vector $z$.
%The latent space is modeled as a Gaussian Mixture Model (GMM), each Gaussian representing a discrete disparity label.
%Thus, each mixture component assigns a likelihood
%\begin{equation}
%    p(x | y) = p(z = f_w(x) | y) |\det J_w(x)|
%\end{equation}
%to the input light field.
%This can be computed accurately due to the tractable Jacobian determinant $J_w(x)$ of the INN.
%Assuming the prior disparity distribution $p(y)$ is uniform, we can infer the posterior distribution
%\begin{equation}
%    p(y | x) = \frac{p(x | y) p(y)}{\sum_{y'}p(x|y')p(y')}
%\end{equation}
%using Bayes rule.
%We train our INN using the Information-Bottleneck loss
%\begin{equation}
%    \mathcal{L}_\mathit{IB} = I(X, Z) - \beta I(Y, Z)
%    \label{eq:loss_ib}
%\end{equation}
%which minimizes the mutual information $I(X, Z)$ between input light field and latent space which forces the network to ignore information unnecessary for the task.
%At the same time it optimizes for the right disparity $y$ by maximizing the mutual information between the network output $z$ in latent space and the disparity label $y$.
%The Lagrange multiplier $\beta$ controls the trade-off between those contradictory goals.
%We present an ablation task regarding the choice of $\beta$ in \cref{sec:ablations}.
%We refer to~\cite{Ardizzone2020} for further details.

%Although, this method underlays the architectural constraints of INNs, it accurately predicts multiple depth modes, within one forward pass.

\subsection{Dataset Generation}
\begin{figure}[t]
    \centering
    \begin{subfigure}{0.325\linewidth}
        \includegraphics[width=\textwidth, trim=0 0 0 80, clip]{figures/dataset/center.png}
        \subcaption{
            Exemplary scene
        }
    \end{subfigure}
    \begin{subfigure}{0.325\linewidth}
        \includegraphics[width=\textwidth, trim=0 0 0 80, clip]{figures/dataset/disp_00.png}
        \subcaption{
            First disparity
        }
    \end{subfigure}
    \begin{subfigure}{0.325\linewidth}
        \includegraphics[width=\textwidth, trim=0 0 0 80, clip]{figures/dataset/disp_01.png}
        \subcaption{
            Second disparity
        }
    \end{subfigure}
    \caption{
        An exemplary scene (a) from our randomly generated dataset. (b) and (c)  show different disparity modes.
        Each pixel has at least one disparity mode.
        Behind semi-transparent objects and at depth edges, a second disparity mode (c) exists.
    }
    \label{fig:dataset}
    \vspace{-3mm}
\end{figure}
To train and validate all methods above, ground truth multimodal depth data is required.
Because all previous light field datasets only contain a single depth per pixel, we generated a novel multimodal depth light field dataset containing 110 randomly generated indoor scenes (see \cref{fig:dataset}).
To improve the training performance, the dataset generator follows four goals: \textit{(i)} relatively photorealistic appearance, \textit{(ii)} high diversity to improve generalization of trained models, \textit{(iii)} many occlusions and depth edges to improve the performance at object edges and, \textit{(iv)} a large proportion of pixels with multiple valid depths.
Note, that we decided to not include reflections explicitely.
However, as~\cite{sinha2012image} demonstrates, reflections at flat surfaces behave similar to alpha-transparency.
Therefore, the methods trained with our dataset should also be usable to estimate multimodal depths caused by reflections.
We refer to~\cref{sec:dataset_generation} for more information on the dataset generation process.

==> Towards Multimodal Depth Estimation from Light Fields/sections/related_work.tex <==
% !TEX root = ../paper.tex
In this section, we first discuss the related methods for depth estimation from light fields.
We secondly introduce different posterior prediction methods mainly inspired by works on uncertainty quantification.

\subsection{Light Field and Multimodal Depth Estimation}
% Oldest method
%In 1987, Bolles \etal~\cite{Bolles1987} have pioneered the topic of depth estimation from light fields.
%The method they proposed utilizes a moving camera mounted on a robot for rendering a three-dimensional image of a static scene.
%Those images can be interpreted as a discrete lightfield with just one angular dimension.
%Their work was the first to introduce and analyze EPIs.
%The authors discovered, described and proofed linear local features in EPI, corresponding to disparity values.
%In order to extract linear features, the proposed algorithm detects edges, peaks and troughs in the epipolar geometry.
%This step is performed by taking the second derivative along the spatial dimension and finding its zero-crossings.
%Lines are fitted along those features and merged with colinear detections for further outlier removal.
%This costly, but intuitive algorithm is able to detect local disparity values for given objects.
%However, the obtained results by the authors are of sparse nature and only present in highly structured areas, due to the inaccurate calibration and low frame-rate of the utilized imaging sensor.
%Over the next decades, light field imaging hardware has evolved massively, yielding towards smaller and more accurate sensors and camera arrays.
%This enabled a constantly improving depth acurracy and made the challange much more prominent.

% Robust Principal Component Analysis
%Heber and Pock~\cite{Heber2014} applied RPCA to light field depth estimation.
%Their method measures the quality of image alignments by projecting images to column vectors of a shared matrix, followed by a convex optimization of stereo matching and denoising.
%To achieve this vectorization, arbitrary views are warped to a predefined coordinate in the center view.
%A convex approximation of RPCA splits a matrix into a sum of two matrices.
%It is based on the observation, that most measurements are a combination of the hidden model in a low dimensional subspace and noise.
%As the problem of finding this partition is NP hard, the authors derived a convex approxiation.
%It can be interpreted as simultaneous optimization of stereo matching and denoising.
%The optimization also includes a smoothness constraint prefering piecewise linear disparity.
%Although the presented approach is a simple and flexible solution to the problem, it is vulnerable to occlusions and produces strong artifacts at object boundaries.
%However, the method is vulnerable to occlusions.

%Although those problems are equally important for all cameras, there exist many challanges inherent to lenslet cameras.

%Jeon \etal~\cite{Jeon2015} specifically address lenslet cameras, proposing a novel distortion correction.
%In contrast to camera arrays, microlense recordings suffer from additional distortion, noise and blur effects.
%The actual depth estimation is performed using a pixel-wise cost volume inspired by traditional stereo matching techniques which is combined with discrete Fourier transform.
%The method is based on traditional stereo matching, but adapted to the small disparity range inherent to microlens arrays.
%Small image patches are shifted with subpixel accuracy by making use of discrete Fourier transform, producing a precisely shifted, reconstructable image.
%For the matching itself, two complementary costs functions:,SAD and GRAD, are utilized.
%Based on the resulting consistency measure, the cost volume containing discrete disparity steps is built.
%To prevent oversmoothing, the authors propose a refinement for sharp occlusion boundaries using an edge preserving filter.
%The resulting cost volume is used as a data model for local disparity estimation.
%However, a global optimization is also required for piecewise smoothness.
%To ensure smoothness, the algorithm applies a sparse matching using graph cut at salient feature points based on SIFT.
%By using those sparse matches, the local cost volumes and an additional smoothness term, the authors proposed a multi-label optimization using graph cut.
%A last refinement step iteratively transfers the discrete depth labels into continuous disparity estimates.
%The method shows a good performance on real images from micro-lense cameras but suffers from noise and artifacts at occlusion boundaries.

%All of the proposals presented so far are based either on EPI analysis or traditional stereo matching algorithms.
%However, the nature of lightfields also allows the production of a focal stack taken at a single point in time.

%Lin \etal~\cite{Lin2015} utilize a focal stack composed of light field data for depth estimation.
%Using the input of lenslet cameras, the focal plane can be shifted arbitrarily in a certain range.
%Their method is based on the local symmetry of the color distribution in a patch around the real depth.
%This observation enables the formulation of a cost function for specific depth labels based on those color distributions.
%While the symmetry property is true for smooth areas, it does not hold at occlusion boundaries.
%Therefore, an accurate distinction between occluded and non-occluded pixels is required.
%This can be achieved using probabilistic reasoning to produce an occlusion probability map.
%In the presence of occlusions the cost function is much more undecided, which leads to the cost variance as a good measure for local occlusion probability.
%To perform global optimization, the authors formulated the problem as a MRF with data and smoothness term.
%Global optimization itself is performed using the graph cut algorithm on multiple image resolutions.
%The proposed method, based on an intermediate focal stack works surprisingly well.
%However, the global optimization takes around 20 minutes and produces only discrete solutions.
%Smoothness is ensured by an optimization with graph cut.
%Unfortunately, the refocusing of micro lense images produces slight artifacts, making the approach not as accurate as most EPI-based methods.

% Structure Tensor
%Wanner and Goldluecke~\cite{Wanner2014} proposed a solution that calculates the disparity directly, using linear algebra operations.
%As the disparity is given by the direction of a line in an EPI, obtaining the slope of this line leads to a good estimate in textured areas.
%To estimate the line slope, an adapted structure tensor is applied to the 4D light field.
%This tensor contains all combinations of partial derivations, integrated over a given area using a Gaussian window function.
%The eigenvector with the strongest eigenvalue of this tensor is aligned with the local gradient of the EPI.
%The strongest eigenvector of this tensor, composed of all partial derivations, is aligned with the EPI gradient.
%In textured areas, this eigenvector is an accurate disparity estimate.
%However, a dense depth estimation requires some optimization method for the untextured areas.
%In addition, the strucure tensor will produce outliers near occlusions, due to different local features in those areas.
%Another problem of locality without further smoothness-constraints is the noise induced by the image sensor and rasterization.
%The proposed global optimization scheme requires a dicretization into depth labels and takes several minutes per image.
%To avoid costly global optimization, the authors also proposed a fast denoising scheme employing \gls{L1}-smoothing.
%Both methods lead to strong artifacts in the results.
%However, due to it's simplicity and robustness, the structure tensor is still a widely used local estimation method.
%As this method produces inaccuracies in non-textured regions and outliers at occlusions, additional optimization methods are required.

% Multiresolution
%Neri \etal~\cite{Neri2015} proposed another method based on $\mathcal{L}^2$ matching costs. 
%A global model is then derived by executing it on multiple image resolutions.
%The method is based on depth samples that are used to map a pixel coordinate from the center view to an arbitrary view in the lightfield.
%An energy for each pair of views is then computed by averaging the difference of \gls{L2} norms of their pixel values, using a moving window.
%The sum of energies over all views is then added to an additional smoothness term.
%In order to model occlusions accordingly, this data term is computed twice for each side of a possible occlusion and the minimal energy is selected.
%The proposed local optimization selects the depth that minimizes the sum of energies over all pairs of views.
%In order to reduce the complexity, a coarse to fine scheme on discrete depth labels is used.
%After computing the confidence measure for each label, a refinement step selects continuous depth values.
%This step is performed iteratively from low to high resolution.
%Therefore, it also provides feasible candidates for smooth regions.
%In order to ensure smoothness, a local optimization of discrete depth labels on a resolution pyramid is performed.
%The method still produces artifacts in large non-textured areas and at object boundaries.

%In general, the estimation near occlusion boundaries is one of the hardest problems of this task.

% Image-Based Rendering for Scenes with Reflections
Sinha \etal~\cite{sinha2012image} separate albedo and reflections in multi-view stereo recordings.
Their method discretizes the disparity space and utilizes a plane-sweep framework to compute an error volume based on pairwise normalized cross correlation.
Up to two distinct layers are extracted from this volume using a modified semi global-matching algorithm.

Johannsen \etal~\cite{johannsen2016sparse} introduced a similar method for multimodal light field depth estimation.
The method uses a dictionary of small EPI patches to encode light fields and estimate the depth at each pixel.
% Each patch corresponds to a distinct disparity and thus can also be used to estimate the depth at each pixel.
In addition, a mask that separates unimodal from bimodal pixels is computed.
% To the best of our knowledge the aforementioned works are the only methods that estimate multiple depth modes.
Both aforementioned methods are able to estimate multiple depth modes from light fields but can not compete with the overall performance of state-of-the-art deep-learning based frameworks.
We refer to~\cref{sec:additional_experiments} for a comparison.

% Spinning Parallelogram Operator
%Zhang \etal~\cite{Zhang2016} introduced the SPO fitting lines with different slopes through the center pixel of a parallelogram.
%Each line divides the parallelogram in two distinct areas.
%The SPO computes $\chi^2$ differences of color distributions between those areas, used as confidence measure.
%Parameterization of a spinning parallelogram itself is expressed by a weighting function, moving its edges according to the depth candidate.
%Therefore, at occlusions, the distance remains in a local maximum for both possible line directions: the depth of the background and the depth for the occluder.
%Due to different occlusions leading to different estimates for horizontal and vertical EPI, a confidence-based filtering is applied to combine both estimates.
%Ambiguous areas with low variance in the distances have a small confidence.
%To combine the estimates of both EPI, the confidence measure is used to compute a weighted sum.
%In order to fill textureless areas, estimates with high confidence are propagated to untextured areas using a guided filter.
%However, the quality at occlusions still depends on the relative angle between EPI extractions and objects boundaries.

% Multi-Orientation
%Most methods use just two orthogonal EPI, having one obvious flaw.
%Both EPI contain parts of the occluder at edges that are not aligned horizontally or vertically.
%Sheng \etal~\cite{Sheng2017} introduced a method to compensate for this effect, utilizing a bigger set of EPI extracted at arbitrary angles.
%They also introduce a novel depth estimation framework marking possible occlusions first.
%For occlusion reasoning, the algorithm utilizes the variance of depth estimates at different EPI orientations.
%In occluded areas, this variance is higher, due to the presence of the occluding object in some orientations.
%Another clue for the object boundaries is the initial depth map.
%The authors use SPO~\cite{Zhang2016} for this step.
%Using the direction of the derived occlusion boundary, the optimal non-occluded EPI is selected to determine the final depth value.
%In order to obtain this orientation, a compass operator, that is also directly applicable to EPI is used.
%Analogous to the SPO, a circle is split into two semicircles along its diameter at an arbitrary angle, in order to computes the difference of color distributions between those semicircles.
%The authors also utilize an operator similar to SPO but comparing the color distributions between semicircles instead of parallelograms.
%The presented results belong to the best methods regarding occlusion handling.
%However, this method depends on many views which are not present for all application scenarios.
%While this method handles occlusions very well, it depends on a large number of views that are not present in all real applications.

% OBER
%In contrast, Schilling \etal~\cite{Schilling2018} introduced a method that does only depend on a cross input.
%It performs local optimization based on PatchMatch~\cite{Barnes2009}.
%As said before, the approach extracts only horizontal and vertical EPI as the input to an iterative optimization scheme.
%A data term evaluates the color variance along linear feature in the EPI that corresponds to the sampled disparity.
%Occlusions are derived implicitely, making use of previous iterations.
%A pixel is defined as occluded, if the disparity difference with its neighbors exceeds some threshold.
%Occluded parts of the EPI are simply rejected by the data term.
%To ensure smoothness in untextured areas, a regularization term based on a modified bilateral filter is applied.
%Sharp edges are preserved by not considering neighbors with a disparity difference exceeding some threshold.
%PatchMatch uses a set of randomly guessed disparity samples for each pixel.
%In order to propagate good disparity guesses to neighbouring areas, the PatchMatch scheme adds the best disparity of each pixel to the sample set of each neighbor.
%Samples from previous iterations are refined by adding random noise with a small variance.
%As the occlusion model requires a good initialization, a much simpler method based on RANSAC line fits is applied as a pre-processing step.
%This model produces state-of-the-art results on the HCI Light Field Benchmark~\cite{Honauer2016}.
%However, it contains many hand tuned parameters which could probably be improved using a learning-based method.

%As the applications of deep learning in the computer vision field grew, it was also applied to the task of light field depth estimation, in order to overcome handcrafted measures.
% % CNN-FC
% Most traditional depth estimation methods for light fields usually focus on two aspects:
% A data term for local disparity predictions in confident regions and an optimization technique for ambiguous regions.
% Because a hand-tuned data term tends to be error prone, more recent approaches learn it directly from the data:
Heber \etal~\cite{heber2016convolutional} introduced the first deep learning based approach for light field depth estimation.
A neural network predicts the slope of local 2D per-pixel hyper planes.
% %The utilized CNN processes a cross-shaped subset of view points.
In a second optimization step, a disparity map is inferred from the hyperplane parameters.
% %The output can be interpreted as two tensors containing all orientation parameters of the local hyperplane.
Due to noise and inaccurate results in untextured areas, an additional post-processing optimization is required.
% %The authors therefore combined the neural network with a convex energy functional for refinement, using a data and a smoothness term.
% %As the resulting energy is convex, the optimization is trivial, using an iterative algorithm.
% %Despite the simplicity of the model, training is hard due to the lack of lightfield data with accurate ground truth disparity.
% %The authors therefore created a new synthetic dataset, using the raytracing software POV-Ray.
% %All rendered scenes contain randomly arranged objects on random backgrounds, that heavily occlude each other.
% %In addition the generalization is improved by data augmentation, including random changes of color, brightness and additional noise.
The approach is a first step in the direction of learned depth from lightfields, but the results suffer from artifacts and blur which are addressed in their follow-up work~\cite{heber2016u,heber2017neural}.
% In addition the authors also contributed a new randomly generated synthetic dataset.
% However, despite the additional optimization framework, the results suffer from strong artifacts and blur.
% In their follow-up work~\cite{heber2016u,heber2017neural} they addressed those problems by utilizing a U-Net architecture~\cite{ronneberger2015u}.
% This significantly increases the receptive radius of the network, without an increase in the number of parameters.
%The new approach predicts the disparity of whole EPI at once, using a u-shaped architecture.
%The network consists of an encoder and a decoder subnetwork, connected by residual pinhole connections.
%In order to train it, the same synthetic dataset was used.
%The first paper~\cite{Heber201602} shows visual and quantitative improvement, but suffers from streaking artifacts, adressed in~\cite{Heber2017}.

% Trained metrics combination
%Aside from pure deep learning methods, the number of combined machine learning and optimization based approaches is growing rapidly.
%Jeon \etal~\cite{Jeon2018} improved their optimization based method by training the combination of different matching cost metrics.
%Due to their strong focus on the specific issues of micro lens sensors, the distortion estimation and correction step remains unchanged.
%The enhanced method is still based on accurate subpixel matching based on Fourier Transform.
%However, the key modification lies in the combination of matching costs.
%In order to cover as much local scene configurations as possible, the authors made use of different consistency measures:
%SAD computes a sum of the \gls{L1} loss over a fixed window.
%The fundamental different ZNCC outputs the cross-correlation after subtracting the mean of a surrounding window.
%Census Transform encodes local image structures using vectorization and GRAD is used to impose higher weights of different costs at occlusions.
%However, the best combination of those consistency cost functions is unknown.
%In order to estimate the best solution to this problem, a learning framework derives an optimal combination by optimizing weights.
%Based on this local estimation, a discrete depth label is selected using random forests.
%A classifying random forest outputs the importance measure for a set containing the most reliable depth values.
%In addition, a regression forest estimates a weighted sum over all candidates to ensure a continuous depth prediction.
%As the forests output a noisy estimate, it is refined by post processing using a median filter.
%The algorithm is trained on 16 scenes from the HCI 4D Lightfield Dataset~\cite{Honauer2016}.
%Because the method aims to perform well for lenslet images, a data augmentation step adapts the input images to this domain.
%The authors proof, that learned matching costs further improve the task of depth estimation in real images.
%However, a huge number of inaccuracies in occluded areas and low textured regions remains.

% EPINet
Shin \etal~\cite{shin2018epinet} use a fully-convolutional architecture for direct disparity regression, consisting of two parts:
A multi-stream network comprised of four input networks for the horizontal, vertical and both diagonal light field view stacks.
The output features of those streams are concatenated and refined by a fully-convolutional head that directly outputs disparities.
%One consists of two convolutional layers, followed by a ReLU and one BN.
%The results of t are then processed by a second CNN part.
%In order to enable end-to-end training, the last layer of the network outputs the disparity directly for each pixel.
%Again, the HCI 4D Lightfield dataset was used to train the proposed architecture.
%However, due to the limited number of scenes in the dataset it was heavily augmented.
%The most involved augmenation step, increases the scene orientation by using only $7 \times 7$ from the $9 \times 9$ views.
%With the additional number of views, the lightfield can be shifted accordingly.
%In addition, there are more common augmentation steps, such as rotation, flipping, image and color scaling, as well as, random adjustments to contrast and brightness.
% TODO: downsides of EPINet
EPI-Net achieves state-of-the-art performance on the HCI 4D Light Field Benchmark~\cite{honauer2016dataset} but is limited to a small disparity interval due to its small receptive field.

% EPI-Shift
Leistner~\etal \cite{leistner2019learning} addressed the problem of light field depth estimation for high resolution and wide baseline light fields utilizing neural networks.
Instead of increasing the receptive field of the network which would yield worse generalization, they proposed to transform the input images with a shear transformation, called EPI-Shift.
The method applies a certain number of forward passes with shifted input EPIs and joins the result into a single prediction.

% Attention based
The most recent works by Tsai \etal~\cite{tsai2020attention} and Chen \etal~\cite{chen2021attention} aim for a better utilization of the light field data.
In contrast to previous methods, they utilize all light field views but fuse them in an early stage to reduce redundancy.

% NeRF
With Neural Radiance Fields (NeRF) Mildenhall \etal~\cite{mildenhall2020nerf} started a new line of research that represents the plenoptic function of a given scene as a neural network.
The network is trained using images recorded from different view points.
At first glance, the radiance along a ray in the NeRF framework also models a depth posterior distribution.
However, we argue that this assumption does not hold in general.
Zhang \etal~\cite{zhang2020nerf++} observed an inherent shape-radiance ambiguity in NeRF models.
This is a caused by training with a photometric loss only instead of supervised learning using ground truth depth.
As a consequence, there exists a family of radiance fields which perfectly explain all training images, even if the shape is incorrect.

% SMD-Nets
Tosi \etal~\cite{tosi2021smd} addressed the problem of smoothness bias at depth discontinuities for stereo depth estimation methods. Their method predicts a bimodal Laplacian mixture distribution for each pixel and always chooses the mode with the largest probability density to retain sharp edges.

%\subsection{Unimodal Posterior Prediction}
\subsection{Prediction of Regression Posteriors}
Traditional depth estimation methods predict a single depth value per pixel.
In the following, we therefore highlight works, focused on other tasks, that estimate a whole posterior instead.
MacKay~\cite{mackay1992practical} introduced the idea of Bayesian Neural Networks (BNNs) by proposing a probabilistic interpretation of the training process.
Instead of predicting only one output, the proposed network models the likelihood of possible outputs given the input.
The posterior probability of network weights, given the dataset can be inferred by maximizing this likelihood.
Now, Bayes rule is applied using maximum likelihood and some prior distribution over the network weights.
However, for large networks, this cannot be computed efficiently.

Neal~\cite{neal2012bayesian} introduced the Markov Chain Monte Carlo (MCMC) method to approximate the posterior over the model weights.
In addition, he analyzed the importance of the chosen prior over a high number of model weights.
This methods enabled an efficient approximation and therefore the training of BNNs.
However, even recent MCMC approaches are only applicable to a limited number of dimensions.

%In ~\cite{Gal2016} Gal and Ghahramani approximate a Gaussian Process by utilizing dropout \todoRM{cite Hinton paper}.
%In order to capture epistemic uncertainty, they propose a new approximation of the marginalisation over all possible networks.
%They show that performing several forward passes with dropout enabled approximates a Bayesian neural networks.
%This is achieved with Monte-Carlo integration by interpreting dropout during a forward pass as a sample from the posterior distribution of all networks.
%In contrast to predictive models with an explicit variance output quantifying the uncertainty, this Monte-Carlo-Dropout technique also captures uncertainty %inherent in the model itself caused by a lack of training data.

Kendall and Gal~\cite{kendall2017uncertainties} analyzed different types of uncertainty relevant for Computer Vision.
They propose to capture aleatoric uncertainty (uncertainty inherent in the data) by training the network to predict a variance for its output.
%This is done by modeling a normal distribution over the outputs. and can also be interpreted as learned loss attenuation.
Epistemic uncertainty (uncertainty inherent in the model), which can be explained away using an infinite amount of data, is inferred using the Monte-Carlo Dropout technique~\cite{gal2016dropout}.
The authors propose a single model to infer both types of uncertainties. % and conclude that those are helpful but not mutually exclusive.

Ilg~\etal~\cite{ilg2018uncertainty} compared different uncertainty quantification methods for optical flow.
They compare aleatoric uncertainty learned by a single network to an ensemble of such networks and further, to a single network with multiple heads trained by the Winner-Takes-it-All loss.
In comparison, the authors find that Monte-Carlo Dropout does not work well for regression tasks and that ensembling also does not provide significantly better uncertainties than single networks.
However, we argue that this is caused by the lack of epistemic uncertainty for optical flow, due to the utilized synthetic datasets being quite large.
As shown by~\cite{kendall2017uncertainties}, Monte Carlo dropout ensembles capture epistemic uncertainty, which can be explained away given enough data.
Because epistemic uncertainty should be close to zero for huge synthetic datasets as used by~\cite{ilg2018uncertainty}, there is no room for improvement over a single network in the first place.

%Ardizzone~\etal~\cite{Ardizzone2019} proposed the utilization of Invertible Neural Networks (INNs) to estimate the posterior distribution over the prediction of a neural network.
%This is achieved by training the often well-defined inverse function that maps the desired outputs to the inputs and some latent space that captures all the information that is not part of the input.
%By forcing the latent space to follow a multivariate Gaussian distribution the posterior can be approximated by sampling from the latent space when performing the forward pass.
%
%In~\cite{Ardizzone2020}, the authors utilize the Information Bottleneck (IB) principle for training an INN.
%For the task of image classification, the proposed training scheme accurately models the data likelihood.
%This is achieved by mapping the input image to a Gaussian Mixture Model (GMM) with each Mixture component representing one class label.
%The exact posterior distribution over all classes is then derived using Bayes Rule.
%As this method requires only a single forward pass, it is much more time efficient than most Bayesian deep learning frameworks.

==> figures/architectures/ib-inn.tex <==
\begin{tikzpicture}[
    data domain/.style={fill=black!20, draw=black, rounded corners=3pt, minimum height=3.15em, minimum width=1.5em, align=center, font=\normalsize},
    fat arrow/.style={double arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=3em, text=black!5},
    unidirectional fat arrow/.style={single arrow, fill=my-gray, draw=black, align=center, text depth=-0.5pt, text width=4em, text=black!5},
    loss/.style={black!75, midway, align=center, font=\footnotesize\sffamily\bfseries}]

    \node [data domain, fill=black!5] (x) {$x$};
    \node [below=6pt of x.south, yshift=5pt] (inp) {\normalsize{\textsc{Light Field}}};

    \node [fat arrow, right=2pt of x.east] (INN) {\textsf{\normalsize{\textbf{INN}}}};

    \node [data domain, right=2pt of INN.east, fill=my-blue!30] (z) {$z$};
    \node [below=6pt of z.south, yshift=5pt] (gmm) {\normalsize{\textsc{GMM}}};
    
    \node [unidirectional fat arrow, right=4pt of z.east] (inference) {\textsf{\scriptsize{\textbf{Bayes Rule}}}};
    
    \node [data domain, right=2pt of inference.east, fill=my-purple!30] (y) {$p(y \! \mid \! x)$};
    \node [below=6pt of y.south, yshift=5pt] (output) {\normalsize{\textsc{Posterior}}};
\end{tikzpicture}


==> figures/bimodality/cnn.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{$1 - \mathrm{\textsc{\textsc{Intersection}}}$},
        xlabel=\scriptsize{\textsc{Fraction of Predicted Pixels}},
        ]
    
        %\addplot[mark=none, black!80, thick] 
        %table[x=frac,y=uncert,col sep=comma] {figures/bimodality/random.csv}; 
        
        \addplot[mark=none, my-orange, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality/bayesian.csv};
        
        \addplot[mark=none, my-purple, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality/discrete.csv};
        
        \addplot[mark=none, my-green, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality/ib-inn.csv}; 

        \addplot[mark=none, black!80, thick, densely dotted]
        table[x=frac,y=oracle,col sep=comma] {figures/bimodality/ib-inn.csv}; 
        
        %\addlegendentry{\scriptsize{Random}}
        \addlegendentry{\scriptsize{ESE}}
        \addlegendentry{\scriptsize{DPP}}
        \addlegendentry{\scriptsize{IB-INN}}
        \addlegendentry{\scriptsize{Oracle}}
    \end{axis}
\end{tikzpicture}


==> figures/bimodality/error.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{\textsc{Bimod. $-$ Oracle}},
        xlabel=\scriptsize{\textsc{Fraction of Predicted Pixels}},
        ]
        
        %\addplot[mark=none, my-blue, thick] 
        %table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality/random.csv}; 

        \addplot[mark=none, my-orange, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality/bayesian.csv}; 
        
        \addplot[mark=none, my-purple, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality/discrete.csv};

        \addplot[mark=none, my-green, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality/ib-inn.csv};
    
        %\addlegendentry{\scriptsize{Random}}
        \addlegendentry{\scriptsize{ESE}}
        \addlegendentry{\scriptsize{DPP}}
        \addlegendentry{\scriptsize{IB-INN}}
        
    \end{axis}
\end{tikzpicture}

==> figures/bimodality_betas/cnn.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        ymin=-0.1,
        ymax=1.6,
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{$1 - \mathrm{\textsc{\textsc{Intersection}}}$},
        xlabel=\scriptsize{\textsc{Fraction of Predicted Pixels}},
        ]
    
        %\addplot[mark=none, black!80, thick] 
        %table[x=frac,y=uncert,col sep=comma] {figures/bimodality/random.csv}; 
        
        \addplot[mark=none, my-orange, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality_betas/0.csv};
        
        \addplot[mark=none, my-purple, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality_betas/1.csv};
        
        \addplot[mark=none, my-green, thick] 
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality_betas/2.csv}; 

        \addplot[mark=none, my-blue, thick]
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality_betas/4.csv}; 
        
        \addplot[mark=none, red!80, thick]
        table[x=frac,y=uncert,col sep=comma] {figures/bimodality_betas/8.csv}; 
        
        \addplot[mark=none, black!80, thick, densely dotted]
        table[x=frac,y=oracle,col sep=comma] {figures/bimodality_betas/8.csv}; 
        
        %\addlegendentry{\scriptsize{Random}}
        \addlegendentry{\scriptsize{$\beta = 0$}}
        \addlegendentry{\scriptsize{$\beta = 1$}}
        \addlegendentry{\scriptsize{$\beta = 2$}}
        \addlegendentry{\scriptsize{$\beta = 4$}}
        \addlegendentry{\scriptsize{$\beta = 8$}}
        \addlegendentry{\scriptsize{Oracle}}
    \end{axis}
\end{tikzpicture}


==> figures/bimodality_betas/error.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.5\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        ymin=-0.1,
        ymax=1.1,
        x label style={at={(axis description cs:0.5,0.0)}},
        y label style={at={(axis description cs:0.05,0.5)}},
        ylabel=\scriptsize{\textsc{Bimod. $-$ Oracle}},
        xlabel=\scriptsize{\textsc{Fraction of Predicted Pixels}},
        ]
        
        \addplot[mark=none, my-orange, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality_betas/0.csv};
        
        \addplot[mark=none, my-purple, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality_betas/1.csv};
        
        \addplot[mark=none, my-green, thick] 
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality_betas/2.csv}; 

        \addplot[mark=none, my-blue, thick]
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality_betas/4.csv}; 
        
        \addplot[mark=none, red!80, thick]
        table[x=frac,y=sparse_err,col sep=comma] {figures/bimodality_betas/8.csv}; 
        
        %\addlegendentry{\scriptsize{Random}}
        \addlegendentry{\scriptsize{$\beta = 0$}}
        \addlegendentry{\scriptsize{$\beta = 1$}}
        \addlegendentry{\scriptsize{$\beta = 2$}}
        \addlegendentry{\scriptsize{$\beta = 4$}}
        \addlegendentry{\scriptsize{$\beta = 8$}}
    \end{axis}
\end{tikzpicture}

==> figures/posteriors/bimodal.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.694\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.2)}},
        y label style={at={(axis description cs:0.2,0.5)}},
        ylabel=$p(y | x)$,
        xlabel=disparity $y$,
        xmin=-1,
        xmax=0.5,
        %ymin=-0.1,
        %ymax=2.1,
        yticklabels={,,},
        xticklabels={,,},
        ]

        \addplot[mark=none, my-green, thick] 
        table[x=y,y=p,col sep=comma] {figures/posteriors/posterior_bm_pred.csv}; 

        \addplot[mark=none, my-orange, thick] 
        table[x=y,y=p,col sep=comma] {figures/posteriors/posterior_bm_inn.csv}; 

        \addlegendentry{\scriptsize{Predictive}}
        \addlegendentry{\scriptsize{IB-INN}}
    \end{axis}
\end{tikzpicture}

==> figures/posteriors/unimodal.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.694\linewidth,
        legend cell align={left},
        legend style={fill=white, fill opacity=0.6, draw opacity=1,text opacity=1, at={(0.02,0.02)},anchor=south west},
        grid=major,
        grid style={densely dotted, gray!50},
        x label style={at={(axis description cs:0.5,0.2)}},
        y label style={at={(axis description cs:0.2,0.5)}},
        ylabel=$p(y | x)$,
        xlabel=disparity $y$,
        xmin=0.0,
        xmax=1.0,
        %ymin=-0.1,
        %ymax=2.1,
        yticklabels={,,},
        xticklabels={,,},
        ]

        \addplot[mark=none, my-green, thick] 
        table[x=y,y=p,col sep=comma] {figures/posteriors/posterior_um_pred.csv}; 

        \addplot[mark=none, my-orange, thick] 
        table[x=y,y=p,col sep=comma] {figures/posteriors/posterior_um_inn.csv};

        \addlegendentry{\scriptsize{Predictive}}
        \addlegendentry{\scriptsize{IB-INN}}
    \end{axis}
\end{tikzpicture}


==> figures/results_posteriors/0007_uni/posteriors.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.422\linewidth,
        legend cell align={left},
        grid=major,
        grid style={densely dotted, gray!50},
        legend style={fill=white, fill opacity=1, draw opacity=1,text opacity=1},
        x label style={at={(axis description cs:0.5,0.07)}},
        y label style={at={(axis description cs:0.07,0.5)}},
        ybar interval,
        % bar width=3,
        ylabel=$p(y | x)$,
        xlabel=discretized disparity $y$,
        xmin=1.5,
        xmax=2.5,
        xticklabels={,,},
        yticklabels={,,},
        ]
        
        \addplot[mark=none, my-orange, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0007_uni/upr.csv};
        
        \addplot[mark=none, my-green, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0007_uni/dpp.csv}; 
        
        \addplot[mark=none, my-blue, fill] 
        table[x=y,y=gt,col sep=comma] {figures/results_posteriors/0007_uni/upr.csv}; 
        
        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{DPP}}
        \addlegendentry{\scriptsize{GT}}
    \end{axis}
\end{tikzpicture}

==> figures/results_posteriors/0123_uni/posteriors.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=0.422\linewidth,
        legend cell align={left},
        grid=major,
        grid style={densely dotted, gray!50},
        legend style={fill=white, fill opacity=1, draw opacity=1,text opacity=1},
        x label style={at={(axis description cs:0.5,0.07)}},
        y label style={at={(axis description cs:0.07,0.5)}},
        ybar interval,
        % bar width=3,
        ylabel=$p(y | x)$,
        xlabel=disparity $y$,
        xmin=1,
        xmax=3.75,
        xticklabels={,,},
        yticklabels={,,},
        ]
        
        \addplot[mark=none, my-orange, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0123_uni/upr.csv};
        
        \addplot[mark=none, my-green, fill] 
        table[x=y,y=p,col sep=comma] {figures/results_posteriors/0123_uni/dpp.csv}; 
        
        \addplot[mark=none, my-blue, fill] 
        table[x=y,y=gt,col sep=comma] {figures/results_posteriors/0123_uni/upr.csv}; 
        
        \addlegendentry{\scriptsize{UPR}}
        \addlegendentry{\scriptsize{DPP}}
        \addlegendentry{\scriptsize{GT}}
    \end{axis}
\end{tikzpicture}
